Structural Constraint Integration in Generative Model for Discovery of Quantum Material Candidates

Billions of organic molecules are known, but only a tiny fraction of the functional inorganic materials have been discovered, a particularly relevant problem to the community searching for new quantum materials. Recent advancements in machine-learning-based generative models, particularly diffusion models, show great promise for generating new, stable materials. However, integrating geometric patterns into materials generation remains a challenge. Here, we introduce Structural Constraint Integration in the GENerative model (SCIGEN). Our approach can modify any trained generative diffusion model by strategic masking of the denoised structure with a diffused constrained structure prior to each diffusion step to steer the generation toward constrained outputs. Furthermore, we mathematically prove that SCIGEN effectively performs conditional sampling from the original distribution, which is crucial for generating stable constrained materials. We generate eight million compounds using Archimedean lattices as prototype constraints, with over 10% surviving a multi-staged stability pre-screening. High-throughput density functional theory (DFT) on 26,000 survived compounds shows that over 50% passed structural optimization at the DFT level. Since the properties of quantum materials are closely related to geometric patterns, our results indicate that SCIGEN provides a general framework for generating quantum materials candidates.

==> archive/m_abstract_240629.tex <==
\begin{abstract}
Compared to the billions of discovered organic molecules, inorganic materials have long faced the challenge of data scarcity, with only a tiny fraction of possible candidates having been discovered. Recent advancements in machine-learning-based generative models, particularly diffusion models, show great promise for generating new, stable materials. However, challenges remain in integrating lattice types into material generation. Here, we introduce Structural Constraint Integration in the GENerative model (SCIGEN). Our system can modify any trained generative diffusion model by strategic masking of the denoised structure with a diffused constrained structure prior to each diffusion step to steer the generation toward constrained outputs. We generate eight million compounds using Archimedean lattices (AL) as prototype constraints, with over 10\% surviving a multi-stage stability pre-screening. High-throughput density functional theory (DFT) on 26,000 survived compounds shows over 50\% passed structural optimization at the DFT level. Since the properties of quantum materials are closely related to the lattice types, SCIGEN provides a general framework for generating quantum materials candidates.
\end{abstract}
\flushbottom
\maketitle
\thispagestyle{empty}

==> archive/m_introduction_240612.tex <==
\section*{Introduction} 
% \input{sections/main_text/m_introduction_memo}
The structure-property relationship is instrumental in understanding quantum and functional materials. Two key structural indicators, symmetry and lattice type, profoundly influence material properties. For example, materials with inversion symmetry can give rise to topological crystalline insulators\autocite{Fu2012TCI}, whereas breaking inversion symmetry can result in a variety of phenomena such as Rashba spin-orbit coupling\cite{Bihlmayer2022Rashba}, ferroelectricity\cite{Martin2017FE}, second harmonic generation\cite{Hung2024SHG}, and topological Weyl semimetals\cite{Armitage2018Weyl}. As to geometry, the lattice type of a material is closely tied to its electronic states and magnetic orderings. The square lattice serves as a prototype for high-temperature cuprate superconductors, while triangular, honeycomb, and kagome lattices can host exotic magnetic states like quantum spin liquids \cite{Savar2017QSL,broholm2020quantum}. Additionally, kagome and Lieb lattices can support electronic flat bands \cite{Kang2020CoSn,slot2017experimental} with technological importance \, and porous structures like zeolites are suitable for catalysis applications. Therefore, identifying new materials with specific symmetries and lattice types is crucial for designing materials with targeted functionalities.

However, there has long been a scarcity of discovered materials. Experimental databases such as the Inorganic Crystal Structure Database (ICSD) and computational databases like the Materials Project contain only a few hundred thousand materials. This is far below the number of possible structures, which grows exponentially with the number of atoms in a unit cell \cite{Oganov2019}. Considering material properties further limits the number of viable candidates. Despite the promising role of quantum spin liquids for quantum computation, only a dozen candidates have been identified after over a decade of intense search\cite{Chamorro2021QSLChem}. For the Lieb lattice, the candidates are even fewer. 

Recently, machine-learning (ML) based materials generators have led to a paradigm shift to design new materials. The conventional approach to material discovery involves proposing potential new structures based on existing ones, such as by substituting atoms in known crystals, followed by evaluating the stability through high-throughput quantum mechanical calculations\cite{kohn1965self}. This method is often a brute-force approach, requiring extensive computational resources. In contrast, ML offers a more efficient alternative by predicting possible atomic substitutions and their resulting stability\cite{kusaba2022crystal, wang2021predicting}. Also, machine learning interatomic potentials (MLIP) behave as the force field accelerating structural optimizations beyond the conventional theoretical optimization methods\cite{chen2022universal, deng2023chgnet, batatia2022mace, riebesell2023matbench}. To explore unseen material structures, diverse representations have been proposed. These include representing structures in high-dimensional spaces\cite{court20203}, graph-based representation\cite{xie2018crystal} and language representations\cite{gruver2024fine}. Such schemes have enabled the discovery of stable material structures that are not present in current databases.

Among the various ML approaches, diffusion-based generative models have shown the most promise in identifying optimal structures\cite{xie2021crystal, yang2023scalable}. These models learn pathways to optimize artificially diffused structures into pristine ones with significant stability and desirable properties. By jointly optimizing crystal lattices, atom types, and atomic coordinates, \textit{ab initio} generation has become feasible\cite{jiao2024crystal}. Initially applied to general material types, generative models have now specialized to discover specific classes of materials, such as semiconductors\cite{wines2023inverse} and metal-organic frameworks (MOFs)\cite{fu2023mofdiff}. The integration of symmetry constraints has further enhanced the performance of generative models, ensuring that the output materials closely resemble those in existing databases\cite{jiao2024space, zeni2023mattergen, cao2024space}. Utilizing Wyckoff positions and crystallographic space groups\cite{aroyo2011crystallography}, these models guide the adjustment of structures to conform to assigned symmetries.

The generative models can propose unseen material structures in quite a short time scale, accelerating the discovery of innovative materials. In particular, Google's GNoME\cite{merchant2023scaling}, which utilizes graph neural networks, predicts 2.2 million new crystalline structures. However, most machine-learning-based generators create new materials from random noise, making it challenging to generate materials with specific lattice constraints. As a result, there is an urgent need to develop a generator capable of producing new materials constrained to particular lattice types, such as kagome lattice materials.

In this work, we have developed Structural Constraint Integration in the GENerative model (SCIGEN). Compared to existing generative models, the work is a new scheme of diffusion-based generative models that allows the incorporation of lattice type and symmetry constraints during the generation. We choose Archimedean lattices\cite{martinez1973archimedean} as the protoype lattices for materials generation. Archimedean lattice is a collection of 11 types of two-dimensional tesselation of the plane where each vertex has the same arrange of polygons. Besides the common square, triangular, honeycomb, and kagome lattices, Archimedean also host other types exotic lattices where no or very few materials examples belong to, including categories with porous structures. In particular, Lieb lattice can be considered as a variation of Archimedean lattice with decorated square lattice. Therefore, materials generation with Archimedean lattice may represent a wide variety of quantum materials such as frustrated magnetism, electronic flat bands, and other applications such as porous structures. 



Inspired by the inpainting method\cite{lugmayr2022repaint, meng2021sdedit} in the image generation field, we have leveraged the structural constraints of Archimedean lattices. We impose the output bulk materials to possess layered structures of geometric patterns of AL formed with magnetic atoms. Our fast down-sampling filters and DFT relaxation verified the existence of stable materials in the generated candidates. To highlight the potential of our work in the condensed matter community, we presented the idea that Lieb lattice materials can have a flat band structure. We intend to guide the model towards generating feasible and experimentally viable materials, addressing the critical gap in the discovery and design of quantum materials. \\





==> archive/m_method_240622.tex <==
\section*{Methods}

\subsection*{Denoising Diffusion Probabilistic Model for periodic crystal generation}

To generate new crystal structures, we utilized an equivariant diffusion-based method, applying the architecture of DiffCSP\cite{jiao2024crystal} as the core of our denoising models. This method enables the \textit{ab initio} generation of crystals by jointly diffusing lattices, fractional coordinates, and atom types, thus allowing these components to influence each other dynamically throughout the generation process. 


The periodic crystals  $\bs{M}$ can be represented by the three components $\bs{M}=(\bs{L}, \bs{F}, \bs{A})$: the fractional coordinates $\bs{F}=\left[\bs{f}_{1}, \bs{f}_{2}, \ldots, \bs{f}_{N}\right] \in \mathbb{R}^{3 \times N}$, the lattice matrix containing three basic vectors $\bs{L}=\left[\bs{l}_{1}, \bs{l}_{2}, \bs{l}_{3}\right] \in \mathbb{R}^{3 \times 3}$, and one-hot representations of atom types $\bs{A}=\left[\bs{a}_{1}, \bs{a}_{2}, \ldots, \bs{a}_{N}\right] \in$ $\mathbb{R}^{h \times N}$. Using these components, the infinite periodic crystal can be described as equation\ref{eq_period_crystal}.

\begin{equation}
\left\{\left(\bs{a}_{i}^{\prime}, \bs{x}_{i}^{\prime}\right) \mid \bs{a}_{i}^{\prime}=\bs{a}_{i}, \bs{x}_{i}^{\prime}=\bs{x}_{i}+\bs{L} \bs{k}, \forall \bs{k} \in \mathbb{Z}^{3 \times 1}\right\}
\label{eq_period_crystal}
\end{equation}


The DiffCSP performs \textit{ab initio} generation of crystal structures by simultaneously diffusing the lattice matrix $\bs{L}$, the fractional coordinate matrix $\bs{F}$, and the atom types $\bs{A}$. $\bs{M}_t=(\bs{L}_t, \bs{F}_t, \bs{A}_t)$ denotes the intermediate state of the crystal structure at time step $t(0 \leq t \leq T)$. The denoising diffusion model consists of the two Markov processes. The first part is the forward diffusion process gradually adding noise to $\bs{M}_{0}$. The second part is the backward denoising process iteratively sampling from the prior distribution $\bs{M}_{T}$ to recover the origin data $\bs{M}_{0}$.  

Since $\bs{L}$ is a continuous variable, diffusion on $\bs{L}$ goes with the Denoising Diffusion Probabilistic Model (DDPM) to train the generative model\cite{ho2020denoising}. We define the forward process that diffuses $\bs{L}_{0}$ towards the prior of the normal distribution $p\left(\bs{L}_{T}\right)=\mathcal{N}(0, \bs{I})$ by $q\left(\bs{L}_{t} \mid \bs{L}_{t-1}\right)$, which can be devised as the probability conditional on the initial distribution (equation \ref{eq_l_noise}). Here, $\beta_{t} \in(0,1)$ is the profile for defining the variance of each diffusion step, and $\bar{\alpha}_{t}=\prod_{s=1}^{t} \alpha_{t}=\prod_{s=1}^{t}\left(1-\beta_{t}\right)$ is designed by the cosine scheduler\cite{nichol2021improved}. 

\begin{equation}
q\left(\bs{L}_{t} \mid \bs{L}_{0}\right)=\mathcal{N}\left(\bs{L}_{t} \mid \sqrt{\bar{\alpha}_{t}} \bs{L}_{0},\left(1-\bar{\alpha}_{t}\right) \bs{I}\right) 
\label{eq_l_noise}
\end{equation}

The backward generation process for the lattice matrix is then defined by equation \ref{eq_l_denoise}, where $\mu\left(\bs{M}_{t}\right)=\frac{1}{\sqrt{\alpha_{t}}}\left(\bs{L}_{t}-\frac{\beta_{t}}{\sqrt{1-\bar{\alpha}_{t}}} \hat{\bs{\epsilon}}_{\bs{L}}\left(\bs{M}_{t}, t\right)\right)$ and $\sigma^{2}\left(\bs{M}_{t}\right)=\beta_{t} \frac{1-\bar{\alpha}_{t-1}}{1-\bar{\alpha}_{t}}$. The denoising term of the lattice matrix $\hat{\bs{\epsilon}}_{\bs{L}}\left(\bs{M}_{t}, t\right) \in \mathbb{R}^{3 \times 3}$ is predicted by the model $\phi\left(\bs{L}_{t}, \bs{F}_{t}, \bs{A}, t\right)$.

\begin{equation}
p\left(\bs{L}_{t-1} \mid \bs{M}_{t}\right)=\mathcal{N}\left(\bs{L}_{t-1} \mid \mu\left(\bs{M}_{t}\right), \sigma^{2}\left(\bs{M}_{t}\right) \bs{I}\right) 
\label{eq_l_denoise}
\end{equation}

The training objective for the denoising processes of the lattice matrix involves minimizing the expected squared difference between the actual noise and the predicted noise across all steps, as shown in the equations below.  

\begin{equation}
\mathcal{L}_{\bs{L}}=\mathbb{E}_{\bs{\epsilon}_{\bs{L}} \sim \mathcal{N}(0, \bs{I}), t \sim \mathcal{U}(1, T)}\left[\left\|\bs{\epsilon}_{\bs{L}}-\hat{\bs{\epsilon}}_{\bs{L}}\left(\bs{M}_{t}, t\right)\right\|_{2}^{2}\right] 
\end{equation}

 Fractional coordinates $\bs{F}$ are a way to specify the positions of atoms within the unit cell of a crystal lattice. These coordinates are expressed as fractions of the unit cell dimensions. The Cartesian coordinates $\bs{X}$ can be derived from the fractional coordinates $\bs{F}$ and the unit cell matrix $\bs{L}$ as $\bs{X} = \bs{L} \bs{F}$. Due to the nature of the periodic boundary condition of crystals, the fractional coordinates are in the form of $[0,1)^{3 \times N}$. The normal distribution used in DDPM does not handle the cyclical and bounded nature of $\bs{F}$. Therefore, we use a Score-Matching (SM) framework with a Wrapped Normal (WN) distribution to address this case\cite{de2022riemannian, song2020improved, song2020score}. During the forward process, we first sample each column of $\bs{\epsilon}_{\bs{F}} \in \mathbb{R}^{3 \times N}$ from $\mathcal{N}(0, \bs{I})$, and then acquire $\bs{F}_{t}=w\left(\bs{F}_{0}+\sigma_{t} \bs{\epsilon}_{\bs{F}}\right)$ where the truncation function $w(\cdot)$ flip the coordinate back to the unit cell. 

\begin{equation}
q\left(\bs{F}_{t} \mid \bs{F}_{0}\right) \propto \sum_{\bs{Z} \in \mathbb{Z}^{3 \times N}} \exp \left(-\frac{\left\|\bs{F}_{t}-\bs{F}_{0}+\bs{Z}\right\|_{F}^{2}}{2 \sigma_{t}^{2}}\right) 
\end{equation}

The backward generation process of fractional coordinates can be written as below, where $\mu_{\bs{F}}\left(\bs{M}_{t}\right)=\frac{1}{\sqrt{\alpha_{t}}}\left(\bs{F}_{t}-\frac{\beta_{t}}{\sqrt{1-\bar{\alpha}_{t}}} \hat{\bs{\epsilon}}_{\bs{F}}\left(\bs{M}_{t}, t\right)\right)$, $\sigma_{\bs{F}}^{2}\left(\bs{M}_{t}\right)=\beta_{t} \frac{1-\bar{\alpha}_{t-1}}{1-\bar{\alpha}_{t}}$. The denoising term $\hat{\bs{\epsilon}}_{\bs{F}}\left(\bs{M}_{t}, t\right) \in \mathbb{R}^{h \times N}$ is predicted by the model $\phi\left(\bs{L}_{t}, \bs{F}_{t}, \bs{A}_{t}, t\right)$.  \\

\begin{equation}
p\left(\bs{F}_{t-1} \mid \bs{M}_{t}\right)=\mathcal{N}\left(\bs{F}_{t-1} \mid \mu_{\bs{F}}\left(\bs{M}_{t}\right), \sigma_{\bs{F}}^{2}\left(\bs{F}_{t}\right) \bs{I}\right),
\end{equation}

The training objective for score matching of fractional coordinates is expressed as an equation below. Here $\lambda_{t}=\mathbb{E}_{\bs{F}_{t}}^{-1}\left[\left\|\nabla_{\bs{F}_{t}} \log q\left(\bs{F}_{t} \mid \bs{F}_{0}\right)\right\|_{2}^{2}\right]$ is approximated via Monte-Carlo sampling.  \\

\begin{equation}
\mathcal{L}_{\bs{F}}=\mathbb{E}_{\bs{F}_{t} \sim q\left(\bs{F}_{t} \mid \bs{F}_{0}\right), t \sim \mathcal{U}(1, T)}\left[\lambda_{t}\left\|\nabla_{\bs{F}_{t}} \log q\left(\bs{F}_{t} \mid \bs{F}_{0}\right)-\hat{\bs{\epsilon}}_{\bs{F}}\left(\bs{M}_{t}, t\right)\right\|_{2}^{2}\right]
\end{equation}

We can represent atom types $\bs{A}$ as the continuous vector of a probability distribution. Diffusion on $\bs{A}$ goes with the DDPM to train the generative model. We define the forward process that diffuses $\bs{A}_{0}$ towards the prior of the normal distribution.   \\

\begin{equation}
q\left(\bs{A}_{t} \mid \bs{A}_{0}\right)=\mathcal{N}\left(\bs{L}_{t} \mid \sqrt{\bar{\alpha}_{t}} \bs{A}_{0},\left(1-\bar{\alpha}_{t}\right) \bs{I}\right) 
\end{equation}

The backward generation process for the atom-type vectors is then defined by the equation below, where $\mu_{\bs{A}}\left(\bs{M}_{t}\right)=\frac{1}{\sqrt{\alpha_{t}}}\left(\bs{A}_{t}-\frac{\beta_{t}}{\sqrt{1-\bar{\alpha}_{t}}} \hat{\bs{\epsilon}}_{\bs{A}}\left(\bs{M}_{t}, t\right)\right), \sigma_{\bs{A}}^{2}\left(\bs{M}_{t}\right)=\beta_{t} \frac{1-\bar{\alpha}_{t-1}}{1-\bar{\alpha}_{t}}$. The denoising term $\hat{\bs{\epsilon}}_{\bs{A}}\left(\bs{M}_{t}, t\right) \in \mathbb{R}^{h \times N}$ is predicted by the model $\phi\left(\bs{L}_{t}, \bs{F}_{t}, \bs{A}_{t}, t\right)$.

\begin{equation}
p\left(\bs{A}_{t-1} \mid \bs{M}_{t}\right)=\mathcal{N}\left(\bs{A}_{t-1} \mid \mu_{\bs{A}}\left(\bs{M}_{t}\right), \sigma_{\bs{A}}^{2}\left(\bs{M}_{t}\right) \bs{I}\right),
\end{equation}

The training objective for the denoising processes of the atom-type vectors involves minimizing the expected squared difference between the actual and predicted noise across all steps, as shown in the equations below.  

\begin{equation}
\mathcal{L}_{\bs{A}}=\mathbb{E}_{\bs{\epsilon}_{\bs{A}} \sim \mathcal{N}(0, \bs{I}), t \sim \mathcal{U}(1, T)}\left[\left\|\bs{\epsilon}_{\bs{A}}-\hat{\bs{\epsilon}}_{\bs{A}}\left(\bs{M}_{t}, t\right)\right\|_{2}^{2}\right] . 
\end{equation}

The overall training objective aims to minimize the difference between the predicted and actual noise vectors across all diffusion steps, with specific objectives defined for each component of the crystal structure:

\begin{equation}
\mathcal{L}_{\bs{M}}=\lambda_{\bs{L}} \mathcal{L}_{\bs{L}}+\lambda_{\bs{F}} \mathcal{L}_{\bs{F}}+\lambda_{\bs{A}} \mathcal{L}_{\bs{A}} . \
\end{equation}


The denoising terms $\hat{\bs{\epsilon}}_{\bs{F}}$, $\hat{\bs{\epsilon}}_{\bs{L}}$, $\hat{\bs{\epsilon}}_{\bs{A}}$ are predicted by the neural network. Built upon EGNN\cite{satorras2021n}, the $s$-th layer message-passing is written as equation\ref{eq_egnn_edge_get}-\ref{eq_egnn_node_update}. Here $\varphi_{m}$ and $\varphi_{h}$ are MLPs. The function $\psi_{\mathrm{FT}}:(-1,1)^{3} \rightarrow[-1,1]^{3 \times K}$ is Fourier Transformation of the relative fractional coordinate $f_{j}-f_{i}$, which transform the value to be coordinate-free.

\begin{align}
\bs{m}_{i j}^{(s)} & =\varphi_{m}\left(\bs{h}_{i}^{(s-1)}, \bs{h}_{j}^{(s-1)}, \bs{L}^{\top} \bs{L}, \psi_{\mathrm{FT}}\left(\bs{f}_{j}-\bs{f}_{i}\right)\right) \label{eq_egnn_edge_get} \\
\bs{m}_{i}^{(s)} & =\sum_{j=1}^{N} \bs{m}_{i j}^{(s)} \label{eq_egnn_edge_sum}\\
\bs{h}_{i}^{(s)} & =\bs{h}_{i}^{(s-1)}+\varphi_{h}\left(\bs{h}_{i}^{(s-1)}, \bs{m}_{i}^{(s)}\right) \label{eq_egnn_node_update}
\end{align}


After $s$ layers of message pass through the fully connected graph, the denoising term on the lattice $\hat{\epsilon}_{L}$ is given by a linear combination of $\bs{L}$, where $\varphi_{L}$ is an MLP with output shape $3 \times 3$.   

\begin{equation}
\hat{\bs{\epsilon}}_{\bs{L}}=\bs{L} \varphi_{L}\left(\frac{1}{N} \sum_{i=1}^{N} \bs{h}_{i}^{(s)}\right)
\end{equation}

The denoising term on the fractional coordinates $\hat{\epsilon}_{F}$ and atom types $\hat{\epsilon}_{A}$ are given as the function of $\bs{h}_{i}^{(s)}$. Here, $\hat{\bs{\epsilon}}_{\bs{F}}[:, i]$ and $\hat{\bs{\epsilon}}_{\bs{A}}[:, i]$ define the $i$-th column of $\hat{\bs{\epsilon}}_{\bs{F}}$ and $\hat{\bs{\epsilon}}_{\bs{A}}$ respectively. $\varphi_{F}$ and $\varphi_{A}$ are MLP on the final representation of these two terms.  

\begin{equation}
\hat{\bs{\epsilon}}_{\bs{F}}[:, i]=\varphi_{F}\left(\bs{h}_{i}^{(s)}\right)
\end{equation}
\begin{equation}
\hat{\bs{\epsilon}}_{\bs{A}}[:, i]=\varphi_{A}\left(\bs{h}_{i}^{(s)}\right)
\end{equation}


\begin{algorithm}
\caption{Training Procedure of DiffCSP}
\begin{algorithmic}[1]
\State \textbf{Input}: lattice matrix $\bs{L}_0$, fractional coordinates $\bs{F}_0$, atom types $\bs{A}_0$, denoising model $\phi$, and the number of sampling steps $T$.
\State Sample $\bs{\epsilon_L} \sim \mathcal{N}(0, I), \bs{\epsilon_F} \sim \mathcal{N}(0, I), \bs{\epsilon_A} \sim \mathcal{N}(0, I)$ and $t \sim \mathcal{U}(1, T)$.
\State $\bs{L}_t \gets \sqrt{\alpha_t}\bs{L}_0 + \sqrt{1 - \alpha_t}\bs{\epsilon_L}$
\State $\bs{F}_t \gets w(\bs{F}_0 + \sigma_t\bs{\epsilon_F})$
\State $\bs{A}_t \gets \sqrt{\alpha_t}\bs{A}_0 + \sqrt{1 - \alpha_t}\bs{\epsilon_A}$
\State $\bs{\hat{\epsilon}_L}, \bs{\hat{\epsilon}_F} , \bs{\hat{\epsilon}_A} \gets \phi(\bs{L}_t, \bs{F}_t, \bs{A}_t, t)$
\State $\mathcal{L}_F \gets \lambda_t\|\nabla_{\bs{F}_t}\log q(\bs{F}_t|\bs{F}_0) - \bs{\hat{\epsilon}_F}\|_2^2$
\State $\mathcal{L}_L \gets \|\bs{\epsilon_L} - \bs{\hat{\epsilon}_L}\|_2^2$
\State $\mathcal{L}_A \gets \|\bs{\epsilon_A} - \bs{\hat{\epsilon}_A}\|_2^2$
\State Minimize $\mathcal{L}_L + \mathcal{L}_F + \mathcal{L}_A$
\end{algorithmic}
\label{alg_train}
\end{algorithm}


% Training Dataset    \\
% MP-20: material structures from the Materials Project database\cite{jain2013commentary} with 20 or less atoms.     \\
% How many materials?  27136 materials in training dataset     \\

Algorithm \ref{alg_train} summarizes the overall algorithm of training DiffCSP. The model is trained on a dataset of over 27,136 material structures sourced from the Materials Project database\cite{jain2013commentary}, which includes a diverse array of crystal structures with less than 20 atoms per unit cell and energy above convex hull lower than 0.08 eV. Supplementary Information 5 presents a more detailed description of the training dataset and statistics. The training process involves the iterative refinement of the model parameters to minimize loss functions associated with each of the structural components ($\bs{L}$, $\bs{F}$, and $\bs{A}$), ensuring the generation of physically and chemically accurate materials.


\subsection*{Inpainting method as a general method for conditional generation}
Inpainting is one of the most well-known methods for guiding the image generation processes. The goal of inpainting is to predict hidden pixels of an image using a mask region as a condition. When the ground-truth image $x$ and the mask $m$ indicating the known region are given, the known pixels are $m \odot x$, and the known pixels are $(1-m) \odot x$. For each reverse step $x_{t}$ to $x_{t-1}$, $x_{t}$ is the input of the denoising score function. Here, we can alter the known regions $m \odot x_{t}$ as long as the properties of the intermediate image $x_{t}$ belong to the corresponding distribution. This allows us to sample the known regions $m \odot x_{t}$ at any time step $t$ of the forward process defined by a Markov Chain of added Gaussian noise. Thus, by combining the known and known regions of similar noise levels, we can guide the denoising step from $x_{t}$ to $x_{t-1}$ given the masked region. RePaint\cite{lugmayr2022repaint} used the expression in equation\ref{eq_repaint_known}-\ref{eq_repaint_combine} for the denoising process.


\begin{align}
x_{t-1}^{\text {c}} & \sim \mathcal{N}\left(\sqrt{\bar{\alpha}_{t}} x_{0},\left(1-\bar{\alpha}_{t}\right) \mathbf{I}\right)    \label{eq_repaint_known} \\
x_{t-1}^{\text {u}} & \sim \mathcal{N}\left(\mu_{\theta}\left(x_{t}, t\right), \Sigma_{\theta}\left(x_{t}, t\right)\right)    \label{eq_repaint_unknown} \\
x_{t-1} & =m \odot x_{t-1}^{\text {c}}+(1-m) \odot x_{t-1}^{\text {u}}   \label{eq_repaint_combine}
\end{align}

In our endeavor to explore materials with specific geometry requirements, the RePaint algorithm can be applicable to guide the denoising process. We regard the magnetic atoms forming the Archimedean lattice layer as the constraint and the other components of the crystal structure as the free regions. 

\subsection*{Initialize the Archimedean Lattice }
We need a workflow to initialize the condition related to the Archimedean lattice and the whole crystal structure to define the required region of the material structure domains. This initialization process involves four steps: the option of Archimedean lattice, the atom types, and the total number of atoms per unit cell. Supplementary Information 2 provides figures of statistics for this initialization step. 

First, we assign the required geometric domain condition to the crystals. In our SCIGEN approach, we specify one of the Archimedean lattice structures, such as triangular, honeycomb, or Kagome lattice. Each type of Archimedean lattice requires the number of vertices per unit cell and the size of the unit cell, depending on that option. Supplementary Information 1 presents the geometric patterns and the preliminary profiles of all Archimedean lattices and Lieb lattices.

Second, we choose the atom type placed on the vertices of the Archimedean lattice layer assigned above. To observe frustrated magnetism in the generated materials, we specify the magnetic atoms (Mn, Fe, Co, Ni, Ru, Nd, Gd, Tb, Dy, Yb). We can specify these atom types independently from the Archimedean lattice choice above. \\
Third, We sample the possible distances of the nearest-neighbor positions of magnetic atoms forming the Archimedean lattices. For each magnetic atom type, we generated the profile of the bond lengths by sampling the nearest-neighbor distances between the corresponding atoms in the MP-20 dataset\cite{xie2018crystal, jain2013commentary} using CrystalNN\cite{pan2021benchmarking}. To ensure the nearest-neighbor distances do not become significantly close, we cut the minimum lengths by the metallic radii\cite{zachariasen1973metallic} for each atom type The bond length distribution for each magnetic atom type are presented in Supplementary Information 2. 

Finally, the total number of atoms per unit cell $\mathrm{N}$ is sampled. Each of Archimedean lattices has the preferable $\mathrm{N}$ values, considering the difference of the unit cell size relative to the bond lengths. We generated the profile of the $\mathrm{N}$ for each Archimedean lattice type and sampled the value from it. The distribution of the $N$ profile for individual atom types and total statistics for each AL type are displayed in Supplementary Information 2. 

Another thing we need to get for generating each material is the masks ($\bs{m_L}$, $\bs{m_F}$, $\bs{m_A}$), specifying the constraints for the lattice matrix, fractional coordinates, and the atom type. About the lattice matrix $\bs{L}=\left[\bs{l}_{1}, \bs{l}_{2}, \bs{l}_{3}\right] \in \mathbb{R}^{3 \times 3}$, the two lattice vectors $\bs{l}_{1}, \bs{l}_{2}$ specify the shape and the size of the Archimedean lattices, while $\bs{l}_{3}$ does not need to be constrained for this purpose. Therefore, we set $\bs{m_L}$ so that $\bs{l}_{1}$ and $\bs{l}_{2}$ are constrained. As the masks for atomic coordinates and atom types, we give constraints on the atoms as the vertices of AL. Therefore, $\bs{m_F}$ and $\bs{m_A}$ are set 'True' for AL vertice atoms and 'False' for the other unconstrained atoms.  


\subsection*{Integration of constrained and unconstrained components to guide material generation process}

In our approach to material design summarized in Algorithm \ref{alg_matinp}, integration of structural constraints plays a pivotal role in ensuring that certain structural elements, like lattice configurations or specific atomic distributions, adhere closely to predefined parameters. This method effectively blends prescribed structural characteristics with the creative latitude allowed in other aspects of the material's architecture. The integration of inpainting techniques in the image generation field into the crystal generative model involves several key steps:

\noindent\textbf{Add Noise to the Constraint Parts:} Initially, we introduce noise to areas of the structure $\bs{M}_0^c$ to get noised structures $\bs{M}_t^c, t \in [1, T]$ where constraints are specified. This operation is aimed at creating a known pathway for denoising the constrained structures. The unconstrained components of the crystals are guided by this known denoising pathway, which results in the configuration achieving the constrained components existing in the final outputs inherently.  

\noindent\textbf{DiffCSP for Denoising the Unconstrained Parts:} Concurrently, the parts of the structure that are free from these specific constraints undergo a denoising process. This process, facilitated by the DiffCSP model, iteratively refines these regions by methodically reducing the introduced noise, thereby nudging them toward realistic and physically plausible configurations.

\noindent\textbf{Combine the Constrained and Unconstrained Parts:} After processing both parts independently, they are carefully recombined. This combination is critical as it ensures the integrity of the predefined constraints is maintained while integrating seamlessly with the freely generated segments. This method preserves essential structural features and fosters innovation in material design.

These techniques are encapsulated in the following algorithm, which employs a Predictor-Corrector sampling\cite{song2020score} to manage the diffusion process. The transition probabilities for the fractional coordinates during the predictor and corrector ($p_{P}$, $p_{C}$) are formulated to reflect the dual process of prediction followed by correction. 

\begin{align}
p\left(\bs{F}_{t-1} \mid \bs{L}_{t}, \bs{F}_{t}, \bs{A}_{t}\right) & =p_{P}\left(\left.\bs{F}_{t-\frac{1}{2}} \right\rvert\, \bs{L}_{t}, \bs{F}_{t}, \bs{A}_{t}\right) p_{C}\left(\bs{F}_{t-1} \mid \bs{L}_{t-1}, \bs{F}_{t-\frac{1}{2}}, \bs{A}_{t-1}\right), \\
p_{P}\left(\left.\bs{F}_{t-\frac{1}{2}} \right\rvert\, \bs{L}_{t}, \bs{F}_{t}, \bs{A}_{t}\right) & =\mathcal{N}_{w}\left(\left.\bs{F}_{t-\frac{1}{2}} \right\rvert\, \bs{F}_{t}+\left(\sigma_{t}^{2}-\sigma_{t-1}^{2}\right) \hat{\bs{\epsilon}}_{\bs{F}}\left(\bs{L}_{t}, \bs{F}_{t}, \bs{A}_{t}, t\right), \frac{\sigma_{t-1}^{2}\left(\sigma_{t}^{2}-\sigma_{t-1}^{2}\right)}{\sigma_{t}^{2}} \bs{I}\right),     \\
p_{C}\left(\bs{F}_{t-1} \mid \bs{L}_{t-1}, \bs{F}_{t-\frac{1}{2}}, \bs{A}_{t-1}\right) & =\mathcal{N}_{w}\left(\bs{F}_{t-1} \left\lvert\, \bs{F}_{t-\frac{1}{2}}+\gamma \frac{\sigma_{t-1}}{\sigma_{1}} \hat{\bs{\epsilon}}_{\bs{F}}\left(\bs{L}_{t-1}, \bs{F}_{t-\frac{1}{2}}, \bs{A}_{t-1}, t-1\right)\right., 2 \gamma \frac{\sigma_{t-1}}{\sigma_{1}} \bs{I}\right)
\end{align}

Algorithm \ref{alg_matinp} presents a novel sampling procedure designed to generate material structures with structural constraints. The algorithm utilizes a diffusion-based model to iteratively refine lattice, fractional coordinates, and atom types iteratively, ensuring the generated structures cover specific geometry as conditions. The procedure begins by initializing random noise for both unconditioned and conditioned matrices. The conditioned structures are represented by the lattice $\bs{L}^{c}_0$, fractional coordinates $\bs{F}^{c}_0$, and atom types $\bs{A}^{c}_0$, along with the corresponding masks $\bs{\bs{m_L}}$, $\bs{\bs{m_F}}$, and $\bs{\bs{m_A}}$ which enforce the structural constraints like an inpainting process in image generation. The initial unconditioned lattice ($\bs{L}^{u}_T$), fractional coordinates ($\bs{F}^{u}_T$), and atom types ($\bs{A}^{u}_T$) are sampled from a standard normal distribution $\mathcal{N}(0, I)$. Similarly, the conditioned lattice ($\bs{L}^{c}_T$), fractional coordinates ($\bs{F}^{c}_T$), and atom types ($\bs{A}^{c}_T$) are also sampled from the same distribution. At each time step $t$, the fractional coordinates $\bs{F}_t$ are updated by combining the conditioned and unconditioned parts using the mask $\bs{m_F}$, formulated as $\bs{F}_T \gets \bs{\bs{m_F}} \odot \bs{F}^{c}_T + (1-\bs{\bs{m_F}}) \odot \bs{F}^{u}_T$. Similar updates are performed for the lattice $\bs{L}_t$ and atom types $\bs{A}_t$ using their respective masks.

The iterative process begins from the final time step $T$ and proceeds backward to 0. For each time step, random noise $\bs{\bs{\epsilon_F}} \sim \mathcal{N}(0, I)$ is sampled for the fractional coordinates, and the model $\phi$ predicts the noise $\bs{\bs{\hat{\epsilon}_F}}$ based on the current state of the matrices $\bs{L}_t$, $\bs{F}_t$, $\bs{A}_t$, and the time step $t$. The unconditioned coordinates $\bs{F}^{u}_{t-\frac{1}{2}}$ are then updated using the predicted noise, incorporating variance scheduling parameters $\sigma_t$ and $\sigma_{t-1}$. The conditioned fractional coordinates $\bs{F}^{c}_{t-\frac{1}{2}}$ are updated by combining the initial feature matrix $\bs{F}_0$ with newly sampled noise $\bs{\bs{\epsilon_F}'}$. Subsequently, the matrices for the next time step $t-1$ are obtained by recombining the conditioned and unconditioned parts using the masks. This includes updates for the lattice ($\bs{L}_{t-1}$) and adjacency ($\bs{A}_{t-1}$) matrices, calculated with additional variance scheduling parameters $\alpha_t$, $\bar{\alpha_t}$, and $\beta_t$. The process continues iteratively until the initial time step is reached, at which point the refined lattice $\bs{L}_0$, fractional coordinates $\bs{F}_0$, and atom types $\bs{F}_0$ are returned. This ensures that the generated material structures respect the given constraints and exhibit realistic and viable configurations.

This approach effectively integrates structural constraints into the diffusion model, enabling the generation of novel material structures that align with the AL structures as the predefined requirements. Using masks to combine conditioned and unconditioned parts ensures that the constraints are maintained throughout the iterative refinement process, resulting in high-quality material structures suitable for practical applications. 


\begin{algorithm}[H]
    \caption{Structural Constraint Integration in Material Generation Procedure}
    \begin{algorithmic}[1]
        \State \textbf{Input}: Constrained lattice matrix $\bs{L}^{c}_0$, atom types $\bs{A}^{c}_0$, fractional coordinates $\bs{F}^{c}_0$, denoising model $\phi$, and the number of sampling steps $T$, step size of Langevin dynamics $\gamma$.
    % \Procedure{SampleInpaint}{}
        % \State $batch\_size \gets batch.num\_graphs$
        \State $\bs{L}^{u}_T \sim \mathcal{N}(0, I), \bs{F}^{u}_T  \sim \mathcal{N}(0, I), \bs{A}^{u}_T \sim \mathcal{N}(0, I)$
        \State $\bs{L}^{c}_T \sim \mathcal{N}(0, I), \bs{F}^{c}_T  \sim \mathcal{N}(0, I), \bs{A}^{c}_T \sim \mathcal{N}(0, I)$
        \State $\text{Load } \bs{L}^{c}_0, \bs{F}^{c}_0, \bs{A}^{c}_0$
        \State $\text{Load } \bs{m_L}, \bs{m_F}, \bs{m_A}$
        % \State $m^{inv}_L, m^{inv}_F, m^{inv}_A \gets 1-\bs{m_L}, 1-\bs{m_F}, 1-M\bs{m_A}$
        \State $\bs{L}_T \gets \bs{m_L} \odot \bs{F}^{c}_T + (1-\bs{m_L}) \odot \bs{F}^{u}_T$
        \State $\bs{F}_T \gets \bs{m_F} \odot \bs{F}^{c}_T + (1-\bs{m_F}) \odot \bs{F}^{u}_T$
        \State $\bs{A}_T \gets \bs{m_A} \odot \bs{A}^{c}_T + (1-\bs{m_A}) \odot \bs{A}^{u}_T$
        \For{$t = T, \dots, 1$}
            % \State $time\_emb \gets self.time\_embedding(t)$
            % \State $c^{for}_0 \gets \sqrt{\bar{\alpha_t}}$ 
            % \State $c^{for}_1 \gets \sqrt{\bar{1-\alpha_t}}$ 
            % \State $c^{rev}_0 \gets 1/\sqrt{\alpha_t}$ 
            % \State $c^{rev}_1 \gets 1/\sqrt{\alpha_t}, (1-\alpha_t)/\sqrt{\bar{1-\alpha_t}}$ 
            % \State $\bs{\epsilon_L}, \bs{\epsilon_F}, \bs{\epsilon_A} \gets \sim \mathcal{N}(0, I), \mathcal{N}(0, I), \mathcal{N}(0, I)$
            \State $\bs{\epsilon_F} \gets \sim \mathcal{N}(0, I)$
            % \State $\bs{\hat{\epsilon}_L}, \bs{\hat{\epsilon}_F}, \bs{\hat{\epsilon}_A} \gets \phi(\bs{L}_t, \bs{F}_t, \bs{A}_t, t)$
            \State $\_, \bs{\hat{\epsilon}_F}, \_ \gets \phi(\bs{L}_t, \bs{F}_t, \bs{A}_t, t)$
            % \State $\bs{L}^{u}_{t-\frac{1}{2}}, \bs{A}^{u}_{t-\frac{1}{2}} \gets \bs{L}^{u}_{t}, \bs{A}^{u}_{t} $   %!!
            \State $\bs{F}^{u}_{t-\frac{1}{2}} \gets w(\bs{F}_t + (\sigma_{t}^2 - \sigma_{t-1}^2)\bs{\hat{\epsilon}_F} + \frac{\sigma_{t-1}\sqrt{\sigma_{t}^2 - \sigma_{t-1}^2}}{\sigma_{t}}\bs{\epsilon_F})$   %!
            % \State $\bs{\epsilon_L}', \bs{\epsilon_F}', \bs{\epsilon_A}' \gets \sim \mathcal{N}(0, I), \mathcal{N}(0, I), \mathcal{N}(0, I)$
            % \State $\bs{\epsilon_F}' \gets \sim \mathcal{N}(0, I)$
            \State $\bs{\epsilon_F}', \bs{\epsilon_L}', \bs{\epsilon_A}' \sim \mathcal{N}(0, I), \mathcal{N}(0, I), \mathcal{N}(0, I)$
            \State $\bs{L}^{c}_{t} \gets \sqrt{\bar{\alpha_t}} \bs{L}^{c}_0 + \sqrt{1-\bar{\alpha_t}} \bs{\epsilon_L}'$    %!!
            \State $\bs{F}^{c}_{t-\frac{1}{2}} \gets w(\bs{F}^{c}_0 + \sigma_{t}\bs{\epsilon_F}')$
            \State $\bs{A}^{c}_{t} \gets \sqrt{\bar{\alpha_t}} \bs{A}^{c}_0 + \sqrt{1-\bar{\alpha_t}} \bs{\epsilon_A}'$    %!!
            \State $\bs{L}_{t} \gets \bs{m_L} \odot \bs{L}^{c}_{t} + (1-\bs{m_L}) \odot \bs{L}^{u}_{t}$  %!!
            \State $\bs{F}_{t-\frac{1}{2}} \gets \bs{m_F} \odot \bs{F}^{c}_{t-\frac{1}{2}} + (1-\bs{m_F}) \odot \bs{F}^{u}_{t-\frac{1}{2}}$
            \State $\bs{A}_{t} \gets \bs{m_A} \odot \bs{A}^{c}_{t} + (1-\bs{m_A}) \odot \bs{A}^{u}_{t}$  %!!
            
            \State $\bs{\epsilon_L}, \bs{\epsilon_F}, \bs{\epsilon_A} \gets \sim \mathcal{N}(0, I), \mathcal{N}(0, I), \mathcal{N}(0, I)$
            \State $\bs{\hat{\epsilon}_L}, \bs{\hat{\epsilon}_F}, \bs{\hat{\epsilon}_A} \gets \phi(\bs{L}_t, \bs{F}_{t-\frac{1}{2}}, \bs{A}_t, t-1)$
            % \State $d_t \gets \frac{\gamma \sigma_{t-1}^2}{\sigma_{t}^2}$
            \State $\bs{L}^{u}_{t-1} \gets \frac{1}{\sqrt{\alpha_t}}(\bs{L}_t - \frac{\beta_t}{\sqrt{1-\alpha_t}} \bs{\hat{\epsilon}_L}) + \sqrt{\frac{\beta_t(1-\bar{\alpha_t})}{1-\alpha_t}} \bs{\epsilon_L}$
            \State $\bs{F}^{u}_{t-1} \gets w(\bs{F}_{t-\frac{1}{2}} + \frac{\gamma \sigma_{t-1}^2}{\sigma_{1}^2} \bs{\hat{\epsilon}_F} + \sqrt{\frac{2\gamma \sigma_{t-1}^2}{\sigma_{1}^2}}\bs{\epsilon_F})$ %!
            \State $\bs{A}^{u}_{t-1} \gets \frac{1}{\sqrt{\alpha_t}}(\bs{A}_t - \frac{\beta_t}{\sqrt{1-\alpha_t}} \bs{\hat{\epsilon}_A}) + \sqrt{\frac{\beta_t(1-\bar{\alpha_t})}{1-\alpha_t}} \bs{\epsilon_A}$
            \State $\bs{\epsilon_F}', \bs{\epsilon_L}', \bs{\epsilon_A}' \sim \mathcal{N}(0, I), \mathcal{N}(0, I), \mathcal{N}(0, I)$
            \State $\bs{L}^{c}_{t-1} \gets \sqrt{\bar{\alpha_t}} \bs{L}^{c}_0 + \sqrt{1-\bar{\alpha_t}} \bs{\epsilon_L}'$
            \State $\bs{F}^{c}_{t-1} \gets w(\bs{F}^{c}_0 + \sigma_{t}\bs{\epsilon_F}')$
            \State $\bs{A}^{c}_{t-1} \gets \sqrt{\bar{\alpha_t}} \bs{A}^{c}_0 + \sqrt{1-\bar{\alpha_t}} \bs{\epsilon_A}'$
            \State $\bs{L}_{t-1} \gets \bs{m_L} \odot \bs{L}^{c}_{t-1} + (1-\bs{m_L}) \odot \bs{L}^{u}_{t-1}$
            \State $\bs{F}_{t-1} \gets \bs{m_F} \odot \bs{F}^{c}_{t-1} + (1-\bs{m_F}) \odot \bs{F}^{u}_{t-1}$
            \State $\bs{A}_{t-1} \gets \bs{m_A} \odot \bs{A}^{c}_{t-1} + (1-\bs{m_A}) \odot \bs{A}^{u}_{t-1}$


        \EndFor
        \State \Return $\bs{L}_0, \bs{F}_0, \bs{A}_0$.
    % \EndProcedure
    \end{algorithmic}
\label{alg_matinp}
\end{algorithm}


\subsection*{Down-sampling to get stable material structures}
Following the generation of materials constrained by Archimedean Lattice (AL) structures, it becomes essential to evaluate their stability. Due to the high volume of generated candidates—often reaching into the millions—a rapid yet reliable method is necessary to assess stability. MLIP is a tool that calculates the total energy of materials and formation energy faster than DFT. However, it is still insensitive to materials that are out of the distribution. Here, we describe our multi-faceted approach to down-sample materials based on stability criteria.


\subsubsection*{Charge Neutrality}
Materials must be electrically neutral to ensure stability and real-world applicability. We employed the SMACT software\cite{davies2019smact} to evaluate the charge neutrality of generated materials. This process, inspired by methodologies described in the CDVAE paper\cite{xie2021crystal}, ensures that only chemically feasible materials are considered in subsequent steps.


\subsubsection*{Density and Space Occupancy Ratio}
Some generated materials feature densely packed atomic configurations, which are unrealistic in actual crystalline phases. To address this, we compare these materials against a reference dataset (MP-20) to identify and eliminate those with excessively high atom densities. The space occupancy ratio $R_{occ}$ is calculated as follows:

\begin{equation}
R_{occ} = \frac{\sum^{N}_{i=1} \frac{4\pi r_i^3}{3}}{V_{cell}}
\end{equation}

where $r_i$ is the radius of the $i$-th atom and $V_{cell}$ is the volume of the unit cell. Materials in MP-20 observed a similar distribution of $R_{occ}$ that is independent of $N$, as we can find in Supplementary Information 6. Materials with an $R_{occ}$ value exceeding 1.7, a threshold determined by the distribution of $R_{occ}$ in the MP-20 dataset are discarded.

\subsubsection*{Graph Neural Network Classifiers for Stability Evaluation}
To rapidly assess the stability of the remaining material candidates, we utilized graph neural networks (GNNs) based on the E3NN\cite{geiger2022e3nn} framework, designed for their efficiency in handling crystallographic data. We developed two models:

\begin{itemize}
    \item \textbf{GNN for Stability $\Psi_1$:} This model predicts whether a material's energy above the convex hull ($E_{\text{hull}}$) is below a threshold of 0.1 eV, which is indicative of thermodynamic stability. The model was trained using data from the Matbench-discovery\cite{riebesell2023matbench} dataset.

    \item \textbf{GNN for Stability $\Psi_2$:} Recognizing the potential for our model to generate materials that diverge from known stable structures, this classifier distinguishes between pristine and diffused structures. Training data included original structures from the MP-20 dataset and versions with added Gaussian noise, simulating potential inaccuracies in atomic positions during generation. We accept that 1$\%$ diffusion materials are stable, but 5$\%$ diffusion materials are unstable. This model helps ensure that even stable materials are not overly distorted or unrealistic.
\end{itemize}

The two GNN-based classifiers are in simple architecture, but presented high accuracy. We present the confusion matrices of the two models in Supplementary Information 6. The prediction accuracy for the test dataset was 0.83 and 0.99, respectively. 

The four-layered simple down-sampling filters could provide us with an instant tool to evaluate the stability of the generated materials. We argue this stability evaluation is valid, as we observed the materials gain stability as it goes through the denoising process from the noisy structures ($\bs{M}_{T}$) to the pristine ones ($\bs{M}_{0}$). The detail of the stability evaluation over the denoising process is shown in Supplementary Information 6. 


\subsection*{DFT for stability evaluation and structural relaxation}
The candidate models are further evaluated with density functional theory (DFT) for potential structural stability. Due to the high cost of DFT calculations, it is necessary to balance the accuracy and throughput. In the first stage of DFT screening, we choose to use a relatively coarse treatment of the electronic structure to evaluate as many candidates as possible (up to 26,000). Plane-wave DFT calculations were performed using the Vienna Ab initio Simulation Package (VASP)\cite{kresse1996efficient}. The calculation used Projector Augmented Wave (PAW) method\cite{blochl1994projector, kresse1999ultrasoft} to describe the effects of core electrons and Perdew-Burke-Ernzerhof (PBE)\cite{perdew1996generalized} implementation of the Generalized Gradient Approximation (GGA) for the exchange-correlation functional. The energy cutoff was $1.2\cdot\text{max(ENMAX)}$ for the plane-wave basis of the valence electrons. The electronic structure was calculated on $\Gamma$-centered mesh for the unit cell (the grid length density is 5 k-points per 1/nm). The total energy tolerance for electronic energy minimization was 10-6 eV, and the energy criterion for structure optimization was 10-5 eV. The maximum number of steps is 60 for electronic self-consistent calculation and 150 for structural optimization. During the structural relaxation, the symmetry of the crystal is maintained while the cell shape/size and all atomic coordinates are allowed to relax. Non-spin-polarized calculation was employed for this initial screening. A small fraction of models failed the electronic structure calculation, which was terminated by errors. These candidates are considered unstable. For the candidates with completed VASP calculation (either because the energy criterion was reached or the maximum number of relaxation steps was reached), the following quantities are extracted/calculated as indicators of stability: (1) maximum interatomic force after relaxation, (2) initial and final total energy, (3) average changes in lattice constants, (4) average changes in atomic coordinates. These quantities are then analyzed and compared to identify potentially stable candidates worth further and more rigorous evaluations.

\subsection*{Band structure calculation for Lieb lattice materials}
The DFT band structure calculations for Lieb lattice structures were performed using VASP. PAW method and PBE exchange-correlation functional were used for all DFT calculations. The initial electronic structure calculations were performed on a K-point mesh centered at Gamma point with resolved value $k_{mesh}$=0.03$\cdot 2\pi$/$\mathring{\text{A}}$ for each structure. The band structure was subsequently calculated on a high symmetry path generated by the VASPKIT code\cite{wang2021vaspkit}.



\subsection*{Data visualization}
 We used VESTA \cite{momma2011vesta} for visualizing the material structures presented in the main article. For Supplementary Information, we utilized OVITO \cite{stukowski2009visualization} to visualize the material structures. 




==> archive/m_method_240703.tex <==
\section*{Methods}

\subsection*{Denoising Diffusion Probabilistic Model for periodic crystal generation}

Since SCIGEN is a generic framework for any denoising diffusion probabilistic model (DDPM), or diffusion model for short, in this work, we utilize an equivariant diffusion-based method of DiffCSP\cite{jiao2024crystal} as the base model of SCIGEN before applying geometric constraint. The DiffCSP method enables an \textit{ab initio} generation of crystals by jointly diffusing lattices, fractional coordinates, and atom types, thus allowing these components to influence each other dynamically throughout the generation process toward stability. 

The periodic crystals $\bs{M}$ can be represented by the three components $\bs{M}=(\bs{L}, \bs{F}, \bs{A})$: the lattice matrix containing three basis vectors $\bs{L}=\left[\bs{l}_{1}, \bs{l}_{2}, \bs{l}_{3}\right] \in \mathbb{R}^{3 \times 3}$, the fractional coordinates $\bs{F}=\left[\bs{f}_{1}, \bs{f}_{2}, \ldots, \bs{f}_{N}\right] \in [0, 1)^{3 \times N}$, and one-hot representations of atom types $\bs{A}=\left[\bs{a}_{1}, \bs{a}_{2}, \ldots, \bs{a}_{N}\right] \in$ $\{0, 1\}^{h \times N}$. Using these components, the infinite periodic crystal can be described as 

\begin{equation}
\left\{\left(\bs{a}_{i}^{\prime}, \bs{x}_{i}^{\prime}\right) \mid \bs{a}_{i}^{\prime}=\bs{a}_{i}, \bs{x}_{i}^{\prime}=\bs{x}_{i}+\bs{L} \bs{k}, \forall \bs{k} \in \mathbb{Z}^{3 \times 1}\right\}
\label{eq_period_crystal}
\end{equation}


The DiffCSP performs \textit{ab initio} generation of crystal structures by simultaneously diffusing the lattice matrix $\bs{L}$, the fractional coordinate matrix $\bs{F}$, and the atom types $\bs{A}$. $\bs{M}_t=(\bs{L}_t, \bs{F}_t, \bs{A}_t)$ denotes the intermediate state of the crystal structure at time step $t$ $(0 \leq t \leq T)$. The denoising diffusion model consists of the two Markov processes. The first part is the forward diffusion process, which gradually adds noise on $\bs{M}_{0}$ to get $\bs{M}_{T}$. The second part is the backward denoising process, which iteratively samples from the prior distribution $\bs{M}_{T}$ to recover the origin crystal $\bs{M}_{0}$.  

Since $\bs{L}$ is a continuous variable, diffusion on $\bs{L}$ goes directly with the diffusion model to train the generative model\cite{ho2020denoising}. We define the forward process that diffuses $\bs{L}_{0}$ towards the prior of the normal distribution $p\left(\bs{L}_{T}\right)=\mathcal{N}(0, \bs{I})$ by $q\left(\bs{L}_{t} \mid \bs{L}_{t-1}\right)$, which can be devised as the probability conditional on the initial distribution (equation \ref{eq_l_noise}). Here, $\beta_{t} \in(0,1)$ is the profile for defining the variance of each diffusion step, and $\bar{\alpha}_{t}=\prod_{s=1}^{t} \alpha_{t}=\prod_{s=1}^{t}\left(1-\beta_{t}\right)$ is designed by the cosine scheduler\cite{nichol2021improved} 

\begin{equation}
q\left(\bs{L}_{t} \mid \bs{L}_{0}\right)=\mathcal{N}\left(\bs{L}_{t} \mid \sqrt{\bar{\alpha}_{t}} \bs{L}_{0},\left(1-\bar{\alpha}_{t}\right) \bs{I}\right) 
\label{eq_l_noise}
\end{equation}

The backward generation process for the lattice matrix is then defined by equation \ref{eq_l_denoise}, where $\mu\left(\bs{M}_{t}\right)=\frac{1}{\sqrt{\alpha_{t}}}\left(\bs{L}_{t}-\frac{\beta_{t}}{\sqrt{1-\bar{\alpha}_{t}}} \hat{\bs{\epsilon}}_{\bs{L}}\left(\bs{M}_{t}, t\right)\right)$ and $\sigma^{2}\left(\bs{M}_{t}\right)=\beta_{t} \frac{1-\bar{\alpha}_{t-1}}{1-\bar{\alpha}_{t}}$. The denoising term of the lattice matrix $\hat{\bs{\epsilon}}_{\bs{L}}\left(\bs{M}_{t}, t\right) \in \mathbb{R}^{3 \times 3}$ is predicted by the model $\phi\left(\bs{L}_{t}, \bs{F}_{t}, \bs{A}_{t}, t\right)$.

\begin{equation}
p\left(\bs{L}_{t-1} \mid \bs{M}_{t}\right)=\mathcal{N}\left(\bs{L}_{t-1} \mid \mu\left(\bs{M}_{t}\right), \sigma^{2}\left(\bs{M}_{t}\right) \bs{I}\right) 
\label{eq_l_denoise}
\end{equation}

The training loss function for the denoising processes of the lattice matrix involves minimizing the expected squared difference between the actual noise and the predicted noise across all steps, which can be written as 

\begin{equation}
\mathcal{L}_{\bs{L}}=\mathbb{E}_{\bs{\epsilon}_{\bs{L}} \sim \mathcal{N}(0, \bs{I}), t \sim \mathcal{U}(1, T)}\left[\left\|\bs{\epsilon}_{\bs{L}}-\hat{\bs{\epsilon}}_{\bs{L}}\left(\bs{M}_{t}, t\right)\right\|_{2}^{2}\right] 
\end{equation}

 Fractional coordinates $\bs{F}$ specify the positions of atoms within the unit cell of a crystal lattice. These coordinates are expressed as fractions of the unit cell dimensions. The Cartesian coordinates $\bs{X}$ can be derived from the fractional coordinates $\bs{F}$ and the unit cell matrix $\bs{L}$ as $\bs{X} = \bs{L} \bs{F}$. Due to the nature of the periodic boundary condition of crystals, the fractional coordinates are in the form of $[0,1)^{3 \times N}$. The normal distribution used in DDPM does not handle the cyclical and bounded nature of $\bs{F}$. Therefore, we use a Score-Matching (SM) framework with a Wrapped Normal (WN) distribution to address this case\cite{de2022riemannian, song2020improved, song2020score}. During the forward process, we first sample each column of $\bs{\epsilon}_{\bs{F}} \in \mathbb{R}^{3 \times N}$ from $\mathcal{N}(0, \bs{I})$, and then acquire $\bs{F}_{t}=w\left(\bs{F}_{0}+\sigma_{t} \bs{\epsilon}_{\bs{F}}\right)$ where the truncation function $w(\cdot)$ flip the coordinate back to the unit cell. 

\begin{equation}
q\left(\bs{F}_{t} \mid \bs{F}_{0}\right) \propto \sum_{\bs{Z} \in \mathbb{Z}^{3 \times N}} \exp \left(-\frac{\left\|\bs{F}_{t}-\bs{F}_{0}+\bs{Z}\right\|_{F}^{2}}{2 \sigma_{t}^{2}}\right) 
\end{equation}

The backward generation process of fractional coordinates can be written as below, where $\mu_{\bs{F}}\left(\bs{M}_{t}\right)=\frac{1}{\sqrt{\alpha_{t}}}\left(\bs{F}_{t}-\frac{\beta_{t}}{\sqrt{1-\bar{\alpha}_{t}}} \hat{\bs{\epsilon}}_{\bs{F}}\left(\bs{M}_{t}, t\right)\right)$, $\sigma_{\bs{F}}^{2}\left(\bs{M}_{t}\right)=\beta_{t} \frac{1-\bar{\alpha}_{t-1}}{1-\bar{\alpha}_{t}}$. The denoising term $\hat{\bs{\epsilon}}_{\bs{F}}\left(\bs{M}_{t}, t\right) \in \mathbb{R}^{h \times N}$ is predicted by the model $\phi\left(\bs{L}_{t}, \bs{F}_{t}, \bs{A}_{t}, t\right)$.  \\

\begin{equation}
p\left(\bs{F}_{t-1} \mid \bs{M}_{t}\right)=\mathcal{N}\left(\bs{F}_{t-1} \mid \mu_{\bs{F}}\left(\bs{M}_{t}\right), \sigma_{\bs{F}}^{2}\left(\bs{F}_{t}\right) \bs{I}\right),
\end{equation}

The training loss function for Score-Matching of fractional coordinates is expressed as 

\begin{equation}
\mathcal{L}_{\bs{F}}=\mathbb{E}_{\bs{F}_{t} \sim q\left(\bs{F}_{t} \mid \bs{F}_{0}\right), t \sim \mathcal{U}(1, T)}\left[\lambda_{t}\left\|\nabla_{\bs{F}_{t}} \log q\left(\bs{F}_{t} \mid \bs{F}_{0}\right)-\hat{\bs{\epsilon}}_{\bs{F}}\left(\bs{M}_{t}, t\right)\right\|_{2}^{2}\right]
\end{equation}

\noindent where $\lambda_{t}=\mathbb{E}_{\bs{F}_{t}}^{-1}\left[\left\|\nabla_{\bs{F}_{t}} \log q\left(\bs{F}_{t} \mid \bs{F}_{0}\right)\right\|_{2}^{2}\right]$ is approximated via Monte-Carlo sampling.  \\

We can represent atom types $\bs{A}$ as the continuous vector of a probability distribution. Diffusion on $\bs{A}$ goes with the DDPM to train the generative model. We define the forward process that diffuses $\bs{A}_{0}$ towards the prior of the normal distribution.   \\

\begin{equation}
q\left(\bs{A}_{t} \mid \bs{A}_{0}\right)=\mathcal{N}\left(\bs{L}_{t} \mid \sqrt{\bar{\alpha}_{t}} \bs{A}_{0},\left(1-\bar{\alpha}_{t}\right) \bs{I}\right) 
\end{equation}

The backward generation process for the atom-type vectors is then defined by the equation below, where $\mu_{\bs{A}}\left(\bs{M}_{t}\right)=\frac{1}{\sqrt{\alpha_{t}}}\left(\bs{A}_{t}-\frac{\beta_{t}}{\sqrt{1-\bar{\alpha}_{t}}} \hat{\bs{\epsilon}}_{\bs{A}}\left(\bs{M}_{t}, t\right)\right), \sigma_{\bs{A}}^{2}\left(\bs{M}_{t}\right)=\beta_{t} \frac{1-\bar{\alpha}_{t-1}}{1-\bar{\alpha}_{t}}$. The denoising term $\hat{\bs{\epsilon}}_{\bs{A}}\left(\bs{M}_{t}, t\right) \in \mathbb{R}^{h \times N}$ is predicted by the model $\phi\left(\bs{L}_{t}, \bs{F}_{t}, \bs{A}_{t}, t\right)$.

\begin{equation}
p\left(\bs{A}_{t-1} \mid \bs{M}_{t}\right)=\mathcal{N}\left(\bs{A}_{t-1} \mid \mu_{\bs{A}}\left(\bs{M}_{t}\right), \sigma_{\bs{A}}^{2}\left(\bs{M}_{t}\right) \bs{I}\right),
\end{equation}

The training loss function for the denoising processes of the atom-type vectors involves minimizing the expected squared difference between the actual and predicted noise across all steps, as shown in the equation below   

\begin{equation}
\mathcal{L}_{\bs{A}}=\mathbb{E}_{\bs{\epsilon}_{\bs{A}} \sim \mathcal{N}(0, \bs{I}), t \sim \mathcal{U}(1, T)}\left[\left\|\bs{\epsilon}_{\bs{A}}-\hat{\bs{\epsilon}}_{\bs{A}}\left(\bs{M}_{t}, t\right)\right\|_{2}^{2}\right] . 
\end{equation}

The overall loss function aims to minimize the difference between the predicted and actual noise vectors across all diffusion steps, with specific objectives defined for each component of the crystal structure:

\begin{equation}
\mathcal{L}_{\bs{M}}=\lambda_{\bs{L}} \mathcal{L}_{\bs{L}}+\lambda_{\bs{F}} \mathcal{L}_{\bs{F}}+\lambda_{\bs{A}} \mathcal{L}_{\bs{A}} . \
\end{equation}


The denoising terms in all loss functions terms $\hat{\bs{\epsilon}}_{\bs{F}}$, $\hat{\bs{\epsilon}}_{\bs{L}}$, $\hat{\bs{\epsilon}}_{\bs{A}}$ are predicted by neural networks. Built upon EGNN\cite{satorras2021n}, the $s$-th layer message-passing is written as equations \ref{eq_egnn_edge_get}-\ref{eq_egnn_node_update}. Here $\varphi_{m}$ and $\varphi_{h}$ are multilayer perceptrons (MLPs). The function $\psi_{\mathrm{FT}}:(-1,1)^{3} \rightarrow[-1,1]^{3 \times K}$ is Fourier Transformation of the relative fractional coordinate $f_{j}-f_{i}$, which transform the value to be coordinate-free.

\begin{align}
\bs{m}_{i j}^{(s)} & =\varphi_{m}\left(\bs{h}_{i}^{(s-1)}, \bs{h}_{j}^{(s-1)}, \bs{L}^{\top} \bs{L}, \psi_{\mathrm{FT}}\left(\bs{f}_{j}-\bs{f}_{i}\right)\right) \label{eq_egnn_edge_get} \\
\bs{m}_{i}^{(s)} & =\sum_{j=1}^{N} \bs{m}_{i j}^{(s)} \label{eq_egnn_edge_sum}\\
\bs{h}_{i}^{(s)} & =\bs{h}_{i}^{(s-1)}+\varphi_{h}\left(\bs{h}_{i}^{(s-1)}, \bs{m}_{i}^{(s)}\right) \label{eq_egnn_node_update}
\end{align}


After $s$ layers of message pass through the fully connected graph, the denoising term on the lattice $\hat{\epsilon}_{L}$ is given by a linear combination of $\bs{L}$, where $\varphi_{L}$ is an MLP with output shape $3 \times 3$.   

\begin{equation}
\hat{\bs{\epsilon}}_{\bs{L}}=\bs{L} \varphi_{L}\left(\frac{1}{N} \sum_{i=1}^{N} \bs{h}_{i}^{(s)}\right)
\end{equation}

The denoising term on the fractional coordinates $\hat{\epsilon}_{F}$ and atom types $\hat{\epsilon}_{A}$ are given as the function of $\bs{h}_{i}^{(s)}$. Here, $\hat{\bs{\epsilon}}_{\bs{F}}[:, i]$ and $\hat{\bs{\epsilon}}_{\bs{A}}[:, i]$ define the $i$-th column of $\hat{\bs{\epsilon}}_{\bs{F}}$ and $\hat{\bs{\epsilon}}_{\bs{A}}$ respectively. $\varphi_{F}$ and $\varphi_{A}$ are MLP on the final representation of these two terms.  

\begin{equation}
\hat{\bs{\epsilon}}_{\bs{F}}[:, i]=\varphi_{F}\left(\bs{h}_{i}^{(s)}\right)
\end{equation}
\begin{equation}
\hat{\bs{\epsilon}}_{\bs{A}}[:, i]=\varphi_{A}\left(\bs{h}_{i}^{(s)}\right)
\end{equation}


\begin{algorithm}
\caption{Training Procedure of DiffCSP}
\begin{algorithmic}[1]
\State \textbf{Input}: lattice matrix $\bs{L}_0$, fractional coordinates $\bs{F}_0$, atom types $\bs{A}_0$, denoising model $\phi$, and the number of sampling steps $T$.
\State Sample $\bs{\epsilon_L} \sim \mathcal{N}(0, I), \bs{\epsilon_F} \sim \mathcal{N}(0, I), \bs{\epsilon_A} \sim \mathcal{N}(0, I)$ and $t \sim \mathcal{U}(1, T)$.
\State $\bs{L}_t \gets \sqrt{\alpha_t}\bs{L}_0 + \sqrt{1 - \alpha_t}\bs{\epsilon_L}$
\State $\bs{F}_t \gets w(\bs{F}_0 + \sigma_t\bs{\epsilon_F})$
\State $\bs{A}_t \gets \sqrt{\alpha_t}\bs{A}_0 + \sqrt{1 - \alpha_t}\bs{\epsilon_A}$
\State $\bs{\hat{\epsilon}_L}, \bs{\hat{\epsilon}_F} , \bs{\hat{\epsilon}_A} \gets \phi(\bs{L}_t, \bs{F}_t, \bs{A}_t, t)$
\State $\mathcal{L}_L \gets \|\bs{\epsilon_L} - \bs{\hat{\epsilon}_L}\|_2^2$
\State $\mathcal{L}_F \gets \lambda_t\|\nabla_{\bs{F}_t}\log q(\bs{F}_t|\bs{F}_0) - \bs{\hat{\epsilon}_F}\|_2^2$
\State $\mathcal{L}_A \gets \|\bs{\epsilon_A} - \bs{\hat{\epsilon}_A}\|_2^2$
\State Minimize $\lambda_{\bs{L}} \mathcal{L}_{\bs{L}}+\lambda_{\bs{F}} \mathcal{L}_{\bs{F}}+\lambda_{\bs{A}} \mathcal{L}_{\bs{A}}$
\end{algorithmic}
\label{alg_train}
\end{algorithm}


% Training Dataset    \\
% MP-20: material structures from the Materials Project database\cite{jain2013commentary} with 20 or less atoms.     \\
% How many materials?  27136 materials in training dataset     \\

Algorithm \ref{alg_train} summarizes the overall algorithm of training DiffCSP. The model is trained on a dataset of over 27,136 material structures sourced from the Materials Project database\cite{jain2013commentary}, which includes a diverse array of crystal structures with less than 20 atoms per unit cell and energy above convex hull ($E_{hull}$) lower than 0.08 eV. Supplementary Information 5 presents a more detailed description of the training dataset and statistics. The training process involves the iterative refinement of the model parameters to minimize loss functions associated with each of the structural components ($\bs{L}$, $\bs{F}$, and $\bs{A}$), ensuring the generation of physically and chemically ``reasonable'' materials.


\subsection*{Initialization of the Archimedean Lattices }
We need a workflow to initialize the condition related to the Archimedean lattice and the whole crystal structure to define the required region of the material structure domains. This initialization process involves four steps: the option of Archimedean lattice, the atom types, and the total number of atoms per unit cell. Supplementary Information 2 provides figures of statistics for this initialization step. 

First, we assign the required geometric domain condition to the crystals. In our SCIGEN approach, we specify one of the Archimedean lattice structures, such as Triangular, Honeycomb, or Kagome lattice. Each type of Archimedean lattice requires the number of vertices per unit cell and the size of the unit cell, depending on that option. Supplementary Information 1 presents the geometric patterns and the preliminary profiles of all Archimedean lattices and Lieb lattices.

Second, we choose the atom type $\mathcal{A}^c$ placed on the vertices of the Archimedean lattice layer assigned above. To observe frustrated magnetism in the generated materials, we specify the magnetic atoms (Mn, Fe, Co, Ni, Ru, Nd, Gd, Tb, Dy, Yb). We can specify these atom types independently from the Archimedean lattice choice above. \\
Third, We sample the possible distances $d^c$ of the nearest-neighbor magnetic atoms forming the Archimedean lattices. For each magnetic atom type $\mathcal{A}^c$, we generated the profile of the bond lengths by sampling the nearest-neighbor distances between the corresponding atoms in the MP-20 dataset\cite{xie2018crystal, jain2013commentary} using CrystalNN\cite{pan2021benchmarking}. To ensure the nearest-neighbor distances do not become significantly close, we cut the minimum lengths by the metallic radii\cite{zachariasen1973metallic} for each atom type. The bond length distribution for each magnetic atom type are presented in Supplementary Information 2. 

Finally, the total number of atoms per unit cell $\mathrm{N}$ is sampled. Each of Archimedean lattices has the preferable $\mathrm{N}$ values, considering the difference of the unit cell size relative to the bond lengths. We generated the profile of the $\mathrm{N}$ for each Archimedean lattice type and sampled the value from it. The distribution of the $N$ profile for individual atom types and total statistics for each AL type are displayed in Supplementary Information 2. 

Another thing we need to get for generating each material is the masks ($\bs{m_L}$, $\bs{m_F}$, $\bs{m_A}$), specifying the constraints for the lattice matrix, fractional coordinates, and the atom type. About the lattice matrix $\bs{L}=\left[\bs{l}_{1}, \bs{l}_{2}, \bs{l}_{3}\right] \in \mathbb{R}^{3 \times 3}$, the two lattice vectors $\bs{l}_{1}, \bs{l}_{2}$ specify the shape and the size of the Archimedean lattices, while $\bs{l}_{3}$ does not need to be constrained for this purpose. Therefore, we set $\bs{m_L}$ so that $\bs{l}_{1}$ and $\bs{l}_{2}$ are constrained. As the masks for atomic coordinates and atom types, we give constraints on the atoms as the vertices of AL. Therefore, $\bs{m_F}$ and $\bs{m_A}$ are set 'True' for AL vertice atoms and 'False' for the other unconstrained atoms.  


\subsection*{Integration of constrained and unconstrained components to guide materials generation}

In our approach to material design summarized in Algorithm \ref{alg_matinp}, integration of geometrical constraints plays a pivotal role in ensuring that certain structural elements, like lattice configurations or specific atomic distributions, adhere closely to predefined parameters. This method effectively blends prescribed structural characteristics with the creative latitude allowed in other aspects of the material's architecture. Previously, a generative model with constraints has been employed in image generation for image inpainting, such as Repaint method \cite{lugmayr2022repaint}. However, the geometrical pattern constraint for crystal generation is still challenging. The generation of crystal generative model with geometrical constraint involves several key steps:

\noindent\textbf{Add Noise to the Constraint Parts:} Initially, we introduce noise to areas of the structure $\bs{M}_0^c$ to get noised structures $\bs{M}_t^c, t \in [1, T]$ where constraints are specified. This operation is aimed at creating a predefined pathway for denoising the constrained structures. The unconstrained components of the crystals are guided by this known denoising pathway, which results in the configuration achieving the constrained components existing in the final outputs inherently.  

\noindent\textbf{DiffCSP for Denoising the Unconstrained Parts:} Concurrently, the parts of the structure that are free from these specific constraints undergo a denoising process. This process, facilitated by the DiffCSP model, iteratively refines these regions by methodically reducing the introduced noise, thereby nudging them toward realistic and physically plausible configurations.

\noindent\textbf{Combine the Constrained and Unconstrained Parts:} After processing both parts independently, they are carefully recombined. This combination is critical as it ensures the integrity of the predefined constraints is maintained while integrating seamlessly with the freely generated segments. This method preserves essential structural features and fosters innovation in material design.

These techniques are encapsulated in the following algorithm, which employs a Predictor-Corrector sampling\cite{song2020score} to manage the diffusion process. The transition probabilities for the fractional coordinates during the predictor and corrector ($p_{P}$, $p_{C}$) are formulated to reflect the dual process of prediction followed by correction. 

\begin{align}
p\left(\bs{F}_{t-1} \mid \bs{L}_{t}, \bs{F}_{t}, \bs{A}_{t}\right) & =p_{P}\left(\left.\bs{F}_{t-\frac{1}{2}} \right\rvert\, \bs{L}_{t}, \bs{F}_{t}, \bs{A}_{t}\right) p_{C}\left(\bs{F}_{t-1} \mid \bs{L}_{t-1}, \bs{F}_{t-\frac{1}{2}}, \bs{A}_{t-1}\right), \\
p_{P}\left(\left.\bs{F}_{t-\frac{1}{2}} \right\rvert\, \bs{L}_{t}, \bs{F}_{t}, \bs{A}_{t}\right) & =\mathcal{N}_{w}\left(\left.\bs{F}_{t-\frac{1}{2}} \right\rvert\, \bs{F}_{t}+\left(\sigma_{t}^{2}-\sigma_{t-1}^{2}\right) \hat{\bs{\epsilon}}_{\bs{F}}\left(\bs{L}_{t}, \bs{F}_{t}, \bs{A}_{t}, t\right), \frac{\sigma_{t-1}^{2}\left(\sigma_{t}^{2}-\sigma_{t-1}^{2}\right)}{\sigma_{t}^{2}} \bs{I}\right),     \\
p_{C}\left(\bs{F}_{t-1} \mid \bs{L}_{t-1}, \bs{F}_{t-\frac{1}{2}}, \bs{A}_{t-1}\right) & =\mathcal{N}_{w}\left(\bs{F}_{t-1} \left\lvert\, \bs{F}_{t-\frac{1}{2}}+\gamma \frac{\sigma_{t-1}}{\sigma_{1}} \hat{\bs{\epsilon}}_{\bs{F}}\left(\bs{L}_{t-1}, \bs{F}_{t-\frac{1}{2}}, \bs{A}_{t-1}, t-1\right)\right., 2 \gamma \frac{\sigma_{t-1}}{\sigma_{1}} \bs{I}\right)
\end{align}

Algorithm \ref{alg_matinp} presents a novel sampling procedure designed to generate material structures with structural constraints. The algorithm utilizes a diffusion-based model to iteratively refine lattice, fractional coordinates, and atom types iteratively, ensuring the generated structures cover specific geometry as conditions. The procedure begins by initializing random noise for both unconditioned and conditioned matrices. The conditioned structures are represented by the lattice $\bs{L}^{c}_0$, fractional coordinates $\bs{F}^{c}_0$, and atom types $\bs{A}^{c}_0$, along with the corresponding masks $\bs{\bs{m_L}}$, $\bs{\bs{m_F}}$, and $\bs{\bs{m_A}}$ which enforce the structural constraints like an inpainting process in image generation. The initial unconditioned lattice ($\bs{L}^{u}_T$), fractional coordinates ($\bs{F}^{u}_T$), and atom types ($\bs{A}^{u}_T$) are sampled from a standard normal distribution $\mathcal{N}(0, I)$. Similarly, the conditioned lattice ($\bs{L}^{c}_T$), fractional coordinates ($\bs{F}^{c}_T$), and atom types ($\bs{A}^{c}_T$) are also sampled from the same distribution. At each time step $t$, the fractional coordinates $\bs{F}_t$ are updated by combining the conditioned and unconditioned parts using the mask $\bs{m_F}$, formulated as $\bs{F}_T \gets \bs{\bs{m_F}} \odot \bs{F}^{c}_T + (1-\bs{\bs{m_F}}) \odot \bs{F}^{u}_T$. Similar updates are performed for the lattice $\bs{L}_t$ and atom types $\bs{A}_t$ using their respective masks.

The iterative process begins from the final time step $T$ and proceeds backward to 0. For each time step, random noise $\bs{\bs{\epsilon_F}} \sim \mathcal{N}(0, I)$ is sampled for the fractional coordinates, and the model $\phi$ predicts the noise $\bs{\bs{\hat{\epsilon}_F}}$ based on the current state of the matrices $\bs{L}_t$, $\bs{F}_t$, $\bs{A}_t$, and the time step $t$. The unconditioned coordinates $\bs{F}^{u}_{t-\frac{1}{2}}$ are then updated using the predicted noise, incorporating variance scheduling parameters $\sigma_t$ and $\sigma_{t-1}$. The conditioned fractional coordinates $\bs{F}^{c}_{t-\frac{1}{2}}$ are updated by combining the initial feature matrix $\bs{F}_0$ with newly sampled noise $\bs{\bs{\epsilon_F}'}$. Subsequently, the matrices for the next time step $t-1$ are obtained by recombining the conditioned and unconditioned parts using the masks. This includes updates for the lattice ($\bs{L}_{t-1}$) and adjacency ($\bs{A}_{t-1}$) matrices, calculated with additional variance scheduling parameters $\alpha_t$, $\bar{\alpha_t}$, and $\beta_t$. The process continues iteratively until the initial time step is reached, at which point the refined lattice $\bs{L}_0$, fractional coordinates $\bs{F}_0$, and atom types $\bs{F}_0$ are returned. This ensures that the generated material structures respect the given constraints and exhibit realistic and viable configurations. Supplementary Information 3 provides the schematic explanation of The denoising process, as well as the integration of constrained and unconstrained components of material structures. 

This approach effectively integrates structural constraints into the diffusion model, enabling the generation of novel material structures that align with the AL structures as the predefined requirements. Using masks to combine conditioned and unconditioned parts ensures that the constraints are maintained throughout the iterative refinement process, resulting in high-quality material structures suitable for practical applications. 


\begin{algorithm}
    \caption{Structural Constraint Integration in Material Generation Procedure}
    \begin{algorithmic}[1]
        \State \textbf{Input}: Constrained lattice matrix $\bs{L}^{c}_0$, atom types $\bs{A}^{c}_0$, fractional coordinates $\bs{F}^{c}_0$, denoising model $\phi$, and the number of sampling steps $T$, step size of Langevin dynamics $\gamma$.
    % \Procedure{SampleInpaint}{}
        % \State $batch\_size \gets batch.num\_graphs$
        \State $\bs{L}^{u}_T \sim \mathcal{N}(0, I), \bs{F}^{u}_T  \sim \mathcal{N}(0, I), \bs{A}^{u}_T \sim \mathcal{N}(0, I)$
        \State $\bs{L}^{c}_T \sim \mathcal{N}(0, I), \bs{F}^{c}_T  \sim \mathcal{N}(0, I), \bs{A}^{c}_T \sim \mathcal{N}(0, I)$
        \State $\text{Load } \bs{L}^{c}_0, \bs{F}^{c}_0, \bs{A}^{c}_0$
        \State $\text{Load } \bs{m_L}, \bs{m_F}, \bs{m_A}$
        % \State $m^{inv}_L, m^{inv}_F, m^{inv}_A \gets 1-\bs{m_L}, 1-\bs{m_F}, 1-M\bs{m_A}$
        \State $\bs{L}_T \gets \bs{m_L} \odot \bs{F}^{c}_T + (1-\bs{m_L}) \odot \bs{F}^{u}_T$
        \State $\bs{F}_T \gets \bs{m_F} \odot \bs{F}^{c}_T + (1-\bs{m_F}) \odot \bs{F}^{u}_T$
        \State $\bs{A}_T \gets \bs{m_A} \odot \bs{A}^{c}_T + (1-\bs{m_A}) \odot \bs{A}^{u}_T$
        \For{$t = T, \dots, 1$}

            \State $\bs{\epsilon_F} \gets \sim \mathcal{N}(0, I)$
     
            \State $\bs{\hat{\epsilon}_L}, \bs{\hat{\epsilon}_F}, \bs{\hat{\epsilon}_A} \gets \phi(\bs{L}_t, \bs{F}_{t}, \bs{A}_t, t)$
            
            % \State $\bs{L}^{u}_{t-\frac{1}{2}}, \bs{A}^{u}_{t-\frac{1}{2}} \gets \bs{L}^{u}_{t}, \bs{A}^{u}_{t} $   %!!

            \State $\bs{L}^{u}_{t-1} \gets \frac{1}{\sqrt{\alpha_t}}(\bs{L}_t - \frac{\beta_t}{\sqrt{1-\alpha_t}} \bs{\hat{\epsilon}_L}) + \sqrt{\frac{\beta_t(1-\bar{\alpha_t})}{1-\alpha_t}} \bs{\epsilon_L}$
            
            \State $\bs{F}^{u}_{t-\frac{1}{2}} \gets w(\bs{F}_t + (\sigma_{t}^2 - \sigma_{t-1}^2)\bs{\hat{\epsilon}_F} + \frac{\sigma_{t-1}\sqrt{\sigma_{t}^2 - \sigma_{t-1}^2}}{\sigma_{t}}\bs{\epsilon_F})$   %!

            \State $\bs{A}^{u}_{t-1} \gets \frac{1}{\sqrt{\alpha_t}}(\bs{A}_t - \frac{\beta_t}{\sqrt{1-\alpha_t}} \bs{\hat{\epsilon}_A}) + \sqrt{\frac{\beta_t(1-\bar{\alpha_t})}{1-\alpha_t}} \bs{\epsilon_A}$
            
            % \State $\bs{\epsilon_L}', \bs{\epsilon_F}', \bs{\epsilon_A}' \gets \sim \mathcal{N}(0, I), \mathcal{N}(0, I), \mathcal{N}(0, I)$
            % \State $\bs{\epsilon_F}' \gets \sim \mathcal{N}(0, I)$
            \State $\bs{\epsilon_F}', \bs{\epsilon_L}', \bs{\epsilon_A}' \sim \mathcal{N}(0, I), \mathcal{N}(0, I), \mathcal{N}(0, I)$
            \State $\bs{L}^{c}_{t-1} \gets \sqrt{\bar{\alpha}_{t-1}} \bs{L}^{c}_0 + \sqrt{1-\bar{\alpha}_{t-1}} \bs{\epsilon_L}'$    %!!
            \State $\bs{F}^{c}_{t-\frac{1}{2}} \gets w(\bs{F}^{c}_0 + \sigma_{t-1}\bs{\epsilon_F}')$
            \State $\bs{A}^{c}_{t-1} \gets \sqrt{\bar{\alpha}_{t-1}} \bs{A}^{c}_0 + \sqrt{1-\bar{\alpha}_{t-1}} \bs{\epsilon_A}'$    %!!
            \State $\bs{L}_{t-1} \gets \bs{m_L} \odot \bs{L}^{c}_{t-1} + (1-\bs{m_L}) \odot \bs{L}^{u}_{t-1}$  %!!
            \State $\bs{F}_{t-\frac{1}{2}} \gets \bs{m_F} \odot \bs{F}^{c}_{t-\frac{1}{2}} + (1-\bs{m_F}) \odot \bs{F}^{u}_{t-\frac{1}{2}}$
            \State $\bs{A}_{t-1} \gets \bs{m_A} \odot \bs{A}^{c}_{t-1} + (1-\bs{m_A}) \odot \bs{A}^{u}_{t-1}$  %!!
            
            \State $\bs{\epsilon_L}, \bs{\epsilon_F}, \bs{\epsilon_A} \gets \sim \mathcal{N}(0, I), \mathcal{N}(0, I), \mathcal{N}(0, I)$
            % \State $\bs{\hat{\epsilon}_L}, \bs{\hat{\epsilon}_F}, \bs{\hat{\epsilon}_A} \gets \phi(\bs{L}_t, \bs{F}_{t-\frac{1}{2}}, \bs{A}_t, t-1)$
            \State $\_, \bs{\hat{\epsilon}_F}, \_ \gets \phi(\bs{L}_{t-1}, \bs{F}_{t-\frac{1}{2}}, \bs{A}_{t-1}, t-1)$
            
            \State $\bs{F}^{u}_{t-1} \gets w(\bs{F}_{t-\frac{1}{2}} + \frac{\gamma \sigma_{t-1}^2}{\sigma_{1}^2} \bs{\hat{\epsilon}_F} + \sqrt{\frac{2\gamma \sigma_{t-1}^2}{\sigma_{1}^2}}\bs{\epsilon_F})$ %!
            \State $\bs{\epsilon_F}', \bs{\epsilon_L}', \bs{\epsilon_A}' \sim \mathcal{N}(0, I), \mathcal{N}(0, I), \mathcal{N}(0, I)$
            \State $\bs{L}^{c}_{t-1} \gets \sqrt{\bar{\alpha}_{t-1}} \bs{L}^{c}_0 + \sqrt{1-\bar{\alpha}_{t-1}} \bs{\epsilon_L}'$
            \State $\bs{F}^{c}_{t-1} \gets w(\bs{F}^{c}_0 + \sigma_{t-1}\bs{\epsilon_F}')$
            \State $\bs{A}^{c}_{t-1} \gets \sqrt{\bar{\alpha}_{t-1}} \bs{A}^{c}_0 + \sqrt{1-\bar{\alpha}_{t-1}} \bs{\epsilon_A}'$
            \State $\bs{L}_{t-1} \gets \bs{m_L} \odot \bs{L}^{c}_{t-1} + (1-\bs{m_L}) \odot \bs{L}^{u}_{t-1}$
            \State $\bs{F}_{t-1} \gets \bs{m_F} \odot \bs{F}^{c}_{t-1} + (1-\bs{m_F}) \odot \bs{F}^{u}_{t-1}$
            \State $\bs{A}_{t-1} \gets \bs{m_A} \odot \bs{A}^{c}_{t-1} + (1-\bs{m_A}) \odot \bs{A}^{u}_{t-1}$


        \EndFor
        \State \Return $\bs{L}_0, \bs{F}_0, \bs{A}_0$.
    % \EndProcedure
    \end{algorithmic}
\label{alg_matinp}
\end{algorithm}


\subsection*{Down-sampling procedure to retrieve stable material structures}
Following the generation of materials constrained by Archimedean Lattice structures, it becomes essential to evaluate their stability. Due to the high volume of generated candidates—often reaching into the millions—a rapid yet reliable method is necessary to assess stability. MLIP is a tool that calculates the total energy of materials and formation energy faster than DFT. However, it is still insensitive to materials that are out of the distribution. Here, we describe our multi-faceted approach to down-sample materials based on stability criteria.


\subsubsection*{Charge Neutrality}
Materials must be electrically neutral to ensure stability and real-world applicability. We employed the SMACT software\cite{davies2019smact} to evaluate the charge neutrality of generated materials. This process, inspired by methodologies described in the CDVAE paper\cite{xie2021crystal}, ensures that only chemically feasible materials are considered in subsequent steps.


\subsubsection*{Density and Space Occupancy Ratio}
Some generated materials feature densely packed atomic configurations, which are unrealistic in actual crystalline phases. To address this, we compare these materials against a reference dataset (MP-20) to identify and eliminate those with excessively high atom densities. The space occupancy ratio $R_{occ}$ is calculated as follows:

\begin{equation}
R_{occ} = \frac{\sum^{N}_{i=1} \frac{4\pi r_i^3}{3}}{V_{cell}}
\end{equation}

where $r_i$ is the radius of the $i$-th atom and $V_{cell}$ is the volume of the unit cell. Materials in MP-20 observed a similar distribution of $R_{occ}$ that is independent of $N$, as we can find in Supplementary Information 6. We discarded materials with an $R_{occ}$ value exceeding 1.7, a threshold based on the distribution of $R_{occ}$ in the MP-20 dataset.

\subsubsection*{Graph Neural Network Classifiers for Stability Evaluation}
To rapidly assess the stability of the remaining material candidates, we utilized graph neural networks (GNNs) based on the E3NN\cite{geiger2022e3nn, chen2021direct} framework, designed for their efficiency in handling crystallographic data. We developed two models:

\begin{itemize}
    \item \textbf{GNN for Stability classification $\Psi_1$:} This model predicts whether a material's energy above the convex hull ($E_{\text{hull}}$) is below a threshold of 0.1 eV, which is indicative of thermodynamic stability. The model was trained using data from the Matbench-discovery\cite{riebesell2023matbench}.

    \item \textbf{GNN for Stability classification $\Psi_2$:} Recognizing the potential for our model to generate materials that diverge from known stable structures, this classifier distinguishes between pristine and diffused structures. Training data included original structures from the MP-20 dataset and versions with added Gaussian noise, simulating potential inaccuracies in atomic positions during generation. We accept that 1$\%$ diffusion materials are stable, but 5$\%$ diffusion materials are unstable. This model helps ensure that even stable materials are not overly distorted or unrealistic.
\end{itemize}

The two GNN-based classifiers are in simple architecture, but presented high accuracy. We present the confusion matrices of the two models in Supplementary Information 6. The prediction accuracy for the test dataset was 0.83 and 0.99, respectively. 

The four-layered simple down-sampling filters could provide us with an instant tool to evaluate the stability of the generated materials. We argue this stability evaluation is valid, as we observed the materials gain stability as it goes through the denoising process from the noisy structures ($\bs{M}_{T}$) to the pristine ones ($\bs{M}_{0}$). The detail of the stability evaluation over the denoising process is shown in Supplementary Information 6. 


\subsection*{DFT for stability evaluation and structural relaxation}
The candidate models are further evaluated with density functional theory (DFT) for potential structural stability. Due to the high cost of DFT calculations, it is necessary to balance the accuracy and throughput. In the first stage of DFT screening, we choose to use a relatively coarse treatment of the electronic structure to evaluate as many candidates as possible (up to 26,000). Plane-wave DFT calculations were performed using the Vienna Ab initio Simulation Package (VASP)\cite{kresse1996efficient}. The calculation used Projector Augmented Wave (PAW) method\cite{blochl1994projector, kresse1999ultrasoft} to describe the effects of core electrons and Perdew-Burke-Ernzerhof (PBE)\cite{perdew1996generalized} implementation of the Generalized Gradient Approximation (GGA) for the exchange-correlation functional. The energy cutoff was $1.2\cdot\text{max(ENMAX)}$ for the plane-wave basis of the valence electrons. The electronic structure was calculated on $\Gamma$-centered mesh for the unit cell (the grid length density is 5 k-points per 1/nm). The total energy tolerance for electronic energy minimization was $10^{-6}$ eV, and the energy criterion for structure optimization was $10^{-5}$ eV. The maximum number of steps is 60 for electronic self-consistent calculation and 150 for structural optimization. During the structural relaxation, the symmetry of the crystal is maintained while the cell shape/size and all atomic coordinates are allowed to relax. Non-spin-polarized calculation was employed for this initial screening. A small fraction of models failed the electronic structure calculation, which were terminated and the corresponding candidates are considered unstable. For the candidates with completed VASP calculation (either because the energy criterion was reached or the maximum number of relaxation steps was reached), the following quantities are extracted/calculated as indicators of potential stability: (1) maximum interatomic force after relaxation, (2) initial and final total energy, (3) average changes in lattice constants, (4) average changes in atomic coordinates. These quantities are then analyzed and compared to identify potentially stable candidates worth further and more rigorous evaluations.

\subsection*{Band structure calculation for Lieb-like lattice materials}
The DFT band structure calculations for Lieb-like lattice structures were performed using VASP. PAW method and PBE exchange-correlation functional were used for all DFT calculations. The initial electronic structure calculations were performed on a K-point mesh centered at Gamma point with resolved value $k_{mesh}$=0.03$\cdot 2\pi$/$\mathring{\text{A}}$ for each structure. The band structure was subsequently calculated on a high symmetry path generated by the VASPKIT code\cite{wang2021vaspkit}.



\subsection*{Data visualization}
 We used VESTA \cite{momma2011vesta} for visualizing the material structures presented in the main article. For Supplementary Information, we utilized OVITO \cite{stukowski2009visualization} to visualize the material structures. 




==> archive/out_arch.tex <==
\stepcounter{suppNoteCounter}
\section{Generated materials of Archimedean Lattice structures}

- We down-sampled the materials.    \\
- We did DFT for structure relaxation.      \\
- We run 26k materials for DFT, and finally get 10k (?) materials as being stable phases.   \\


% Replace the figure with the ones after DFT relaxation. 

\begin{figure}[H]
\includegraphics[width=0.9\textwidth]{figures/SI_crys_triangular.pdf}
\centering
\caption{
\textbf{Generated materials of a triangular lattice structures} \textbf{a.} xxx
}
\label{SI_crys_triangular}
\end{figure}



\begin{figure}[H]
\includegraphics[width=0.9\textwidth]{figures/SI_crys_honeycomb.pdf}
\centering
\caption{
\textbf{Generated materials of a honeycomb lattice structures} \textbf{a.} xxx
}
\label{SI_crys_honey}
\end{figure}


\begin{figure}[H]
\includegraphics[width=0.9\textwidth]{figures/SI_crys_kagome.pdf}
\centering
\caption{
\textbf{Generated materials of a Kagome lattice structures} \textbf{a.} xxx
}
\label{SI_crys_kagome}
\end{figure}


\begin{figure}[H]
\includegraphics[width=0.9\textwidth]{figures/SI_crys_square.pdf}
\centering
\caption{
\textbf{Generated materials of a square lattice structures} \textbf{a.} xxx
}
\label{SI_crys_square}
\end{figure}


\begin{figure}[H]
\includegraphics[width=0.9\textwidth]{figures/SI_crys_elt.pdf}
\centering
\caption{
\textbf{Generated materials of an elongated triangular lattice structures} \textbf{a.} xxx
}
\label{SI_crys_elt}
\end{figure}


\begin{figure}[H]
\includegraphics[width=0.9\textwidth]{figures/SI_crys_sns.pdf}
\centering
\caption{
\textbf{Generated materials of a snub square lattice structures} \textbf{a.} xxx
}
\label{SI_crys_sns}
\end{figure}


\begin{figure}[H]
\includegraphics[width=0.9\textwidth]{figures/SI_crys_tsq.pdf}
\centering
\caption{
\textbf{Generated materials of a truncated square lattice structures} \textbf{a.} xxx
}
\label{SI_crys_tsq}
\end{figure}


\begin{figure}[H]
\includegraphics[width=0.9\textwidth]{figures/SI_crys_srt.pdf}
\centering
\caption{
\textbf{Generated materials of a small rhombitrihexagonal lattice structures} \textbf{a.} xxx
}
\label{SI_crys_srt}
\end{figure}


\begin{figure}[H]
\includegraphics[width=0.9\textwidth]{figures/SI_crys_snh.pdf}
\centering
\caption{
\textbf{Generated materials of a snub hexagonal lattice structures} \textbf{a.} xxx
}
\label{SI_crys_snh}
\end{figure}


\begin{figure}[H]
\includegraphics[width=0.9\textwidth]{figures/SI_crys_trh.pdf}
\centering
\caption{
\textbf{Generated materials of a truncated hexagonal lattice structures} \textbf{a.} xxx
}
\label{SI_crys_trh}
\end{figure}


\begin{figure}[H]
\includegraphics[width=0.95\textwidth]{figures/SI_crys_grt.pdf}
\centering
\caption{
\textbf{Generated materials of a great rhombitrihexagonal lattice structures} \textbf{a.} xxx
}
\label{SI_crys_grt}
\end{figure}


% \input{sections/si_text/si_data_tables/data_table_tri}

% \input{sections/si_text/si_data_tables/data_table_hon}

% \input{sections/si_text/si_data_tables/data_table_kag}

% \input{sections/si_text/si_data_tables/data_table_sqr}

% \input{sections/si_text/si_data_tables/data_table_lieb}






==> archive/s_diff_theory.tex <==
\stepcounter{suppNoteCounter}
\section{Diffusion model: a detailed explanation}

XXX







\begin{equation}
q\left(x_{t} \mid x_{t-1}\right)=\mathcal{N}\left(x_{t} ; \sqrt{1-\beta_{t}} x_{t-1}, \beta_{t} \mathbf{I}\right) 
\end{equation}




\begin{equation}
p_{\theta}\left(x_{t-1} \mid x_{t}\right)=\mathcal{N}\left(x_{t-1} ; \mu_{\theta}\left(x_{t}, t\right), \Sigma_{\theta}\left(x_{t}, t\right)\right) 
\end{equation}


\begin{equation}
\mu_{\theta}\left(x_{t}, t\right)=\frac{1}{\sqrt{\alpha_{t}}}\left(x_{t}-\frac{\beta_{t}}{\sqrt{1-\bar{\alpha}_{t}}} \epsilon_{\theta}\left(x_{t}, t\right)\right) 
\end{equation}


\begin{equation}
q\left(x_{t} \mid x_{0}\right)=\mathcal{N}\left(x_{t} ; \sqrt{\bar{\alpha}_{t}} x_{0},\left(1-\bar{\alpha}_{t}\right) \mathbf{I}\right) 
\end{equation}



==> sections/main_text/m_author_contributions.tex <==
\section*{Author Contributions Statement}
\textcolor{todo}{- Write Author contribution section}  \\
RO took the lead in the project. ML designed the project provided supervision and revised the manuscript.


\section*{Competing Interests Statement}
The authors declare no competing interests. 

==> sections/main_text/m_introduction_memo.tex <==
==== Memo =====
[1] Background, Introduction    \\
flustrated magnetism\cite{lacroix2011introduction, ramirez1994strongly, lhotel2020fragmentation, vojta2018frustration, khatua2023experimental}  \\
Quantum spin liquid (QSL)\cite{broholm2020quantum, ma2018recent, shaginyan2020theoretical, vasiliev2018milestones, starykh2015unusual, witczak2014correlated}    \\
QSL candidate materials in nature\cite{inosov2018quantum}     \\
QSL candidates with Kagome lattice and other Archimedean lattices?\cite{yin2022topological, rau2019frustrated, de2019topological} \\
What is QSL, examples like RuCl3    \\
Unique properties of QSL    \\
Structure-property relationship of materials\cite{le2012quantitative}, Unique structures    \\
Triangular, Honeycomb, Kagome, other Archimedean lattice (AL) structures\cite{martinez1973archimedean, eddi2009archimedean, henriksen1962structure}.    \\
Lieb lattice    \\
Unit cell: hexagonal if kagome, honeycomb, triangular.     \\
Magnetic atoms     \\
How to determine if the materials are QSL or not    \\
Magnetic structure: Antiferromagnetic property?\cite{bonbien2021topological}
Susceptibility    \\
neutron scattering  \\
Existing issue: hard to find candidate materials. -> only a few candidates    \\


[2] Material design, generation   \\
Experimental    \\
Try and error, which consume time and resources   \\
Computation-based approach   \\
high-throughout virtual screening (HTVS)\cite{pyzer2015high}   \\
workflow: (1) combinatorially substituting elements in known crystal structures, (2) optimizing the candidate structures using density functional theory (DFT) calculations, and (3) experimental verification.     \\
DFT etc   \\
There are many difficult properties to calculate by DFT (e.g. non-collinear magnetic moment, magnetic structures)   \\
Computational power issue   \\
Machine learning approach: Inverse-design of materials with ML\cite{kim2020inverse, chen2021generative, noh2019inverse, anelli2018generalized, ren2022invertible, hoffmann2019data, wines2023inverse}    \\
Should we mention inverse design, generation of small molecules, protein\cite{okesola2018multicomponent}, etc? 
GNN\cite{zhou2020graph, duvenaud2015convolutional} (CGCNN\cite{xie2018crystal}, E3NN\cite{geiger2022e3nn}, ALIGNN\cite{choudhary2021atomistic}, etc) for Materials property prediction   \\
Magnetic structure\cite{merker2022machine, okabe2023materials}, Phonon DoS\cite{chen2021direct}, phonon bands\cite{okabe2023virtual}, electronic property\cite{zhuo2018predicting}  \\
MLIP: M3GNet\cite{[chen2022universal}, CHGNet\cite{deng2023chgnet}, MACE\cite{batatia2022mace, batatia2023foundation, kovacs2023evaluation}, NequIP\cite{batzner20223}, etc\cite{bartok2018machine},  \\
Matbench-Discovery: material stability, property evaluation\cite{batatia2022mace, batatia2023foundation, kovacs2023evaluation, riebesell2023matbench}  \\    
which can find stable phase and formation energy.    \\
Stability evaluation: energy above the convex hull\cite{bartel2022review, kingsbury2022flexible}   \\
Template method (substitute atoms of existing crystals)   \\
Space group   \\
Generative model    \\
VAE\cite{doersch2016tutorial, }, GAN\cite{goodfellow2020generative, creswell2018generative, mirza2014conditional}, etc   \\
Crystal generation examples\cite{dan2020generative, nouira2018crystalgan, kim2020generative}
LLM-based approach    \\
Crystal generation: CrystalLLM\cite{gruver2024fine}   \\
Space group, symmetry\cite{aroyo2011crystallography}   \\
Symmetric material generation\cite{zhao2023physics}   \\
Element-substitution\cite{kusaba2022crystal}    \\
Diffusion model: DDPM\cite{ho2020denoising}, Score-based DM\cite{song2020score, jo2022score}  \\
Image generation: Stable diffusion, controller, midjourney, etc   \\
Diffusiom model for Graph\cite{liu2023generative, wang2022deep}
Crystal generation: CDVAE\cite{xie2021crystal}, DiffCSP\cite{jiao2024crystal}, DiffCSP++\cite{jiao2024space}, MOFDiff\cite{fu2023mofdiff}, UniMat\cite{yang2023scalable}, GNoMe\cite{merchant2023scaling}, MatterGen\cite{zeni2023mattergen}, etc   \\
Inpainting: guide the denoising diffusion model generation processes.    \\
RePaint\cite{lugmayr2022repaint}, SDEdit\cite{meng2021sdedit}, etc   \\
Inpainting has been applied for molecular generation for binding site conditioning\cite{schneuing2022structure} but has not worked for crystals with specific geometry.     \\

[3] Research goal      \\
In this research, we developed a generative model for producing candidate materials for QSL.    \\
Apply inpainting so that the output crystals have an AL layer with magnetic atoms.    \\
Restraints on fractional coordinates    \\
Filter the outputs based on the stability.   \\
Discovery of Lieb lattice materials\cite{slot2017experimental}  \\
flat bands\cite{kang2020topological, kang2020topological, regnault2022catalogue,}.    \\
Add the generated QSL candidate to the training data   \\
